Modelling heterogeneity in the classification process in multi-species distribution models can improve predictive performance

1. Species distribution models and maps from large-scale biodiversity data are necessary for conservation management. One current issue is that biodiversity data are prone to taxonomic misclassifications. Methods to account for these misclassifications in multispecies distribution models have assumed that the classification probabilities are constant throughout the study. In reality, classification probabilities are likely to vary with several covariates. Failure to account for such heterogeneity can lead to bias in parameter estimates. 2. Here we present a general multispecies distribution model that accounts for heterogeneity in the classification process. The proposed model assumes a multinomial generalised linear model for the classification confusion matrix. We compare the performance of the heterogeneous classification model to that of the homogeneous classification model by assessing how well they estimate the parameters in the model and their predictive performance on hold-out samples. We applied the model to gull data from Norway, Denmark and Finland, obtained from GBIF. 3. Our simulation study showed that accounting for heterogeneity in the classification process increased precision by 30% and reduced accuracy and recall by 6%. Applying the model framework to the gull dataset did not improve the predictive performance between the homogeneous and heterogeneous models due to the smaller misclassified sample sizes. However, when machine learning predictive scores are used as weights to inform the species distribution models about the classification process, the precision increases by 70%. 4. We recommend multiple multinomial regression to be used to model the variation in the classification process when the data contains relatively larger misclassified samples. Machine prediction scores should be used when the data contains relatively smaller misclassified samples.

==> AuthorContribution.tex <==
\section{Author Contribution}
All authors were involved in the idea conception and writing of the manuscript, KPA and RBO were involved with the methodology development, WK ran the ML algorithm and KPA ran the entire analysis used in this paper and led the writing of the manuscript.

==> Chuff.tex <==
It is possible, however, to make use of the classifications from the ML algorithm and build a statistical model that provides uncertainty in the classification probabilities (also known as the confusion matrix). This can be made possible by using the observation confirmation model, which involves selecting a sub-sample of the observation and verification of these observations by an expert \citep{wright2020modelling}. This model provides additional information, the verified data, which makes the estimation of the false positives identifiable like any other occupancy or abundance model \citep{chambert2015modeling, wright2020modelling}. This model to our best of knowledge has not been used in the case where the Machine Learning algorithms serve as experts to confirm the data observed, and our proposed model makes use of these algorithms as experts. This makes it possible to use all samples for the analysis and get more precise estimates.




The model framework, how the model is fit, evaluation of the parameters in the model and prediction of the true species abundance as well as simulation study and application to real data are provided in section 2. In section three we present the results and write discussions in section four. 

\section{Methodology}

\subsection{Model framework}

We consider that over the study region $D \in \mathbb{R}^2$, there are $j = 1, 2, \ldots , R$ indexed presence only locations that have $i=1,2, \ldots, S$ species under study. We assume that each location $j$ has only one of the $S$ species. We assume that these locations are the realisations of the point pattern which is characterised by the mean intensity \citep{cressie2015statistics}, although the model works with other assumptions on the locations. Using the observation confirmation model, we have access to verified data (\textbf{V}) and reported data (\textbf{Y}). The reported data is the data that we obtain from the Citizen Scientist. 

Let $\lambda_{ij}$ be the mean intensity of the verified species $i = 1,2,\ldots, S$ at location $j =1,2,\ldots,R$. The mean intensity can be modelled as an inhomogeneous point process (PPM) which assumes that the data are dependent on the environment covariate,  or as a log-Cox Gaussian Point process (LGCP) where we assume a spatial dependency in the observed data \citep{renner2015point}. The mean intensity of the verified observations \textbf{V} was modelled as a log-Gaussian Cox process with the mean intensity $\lambda_{ij}$. That is;

\begin{equation}
 \ln (\lambda_{ij})= \beta_{0i} +  \beta'_{1i}  \textbf{x} + \xi  ,
\end{equation}
where $\beta_{0i}$ is the intercept of species $i$, $\beta_{1i}$ is the covariate effect, $\textbf{x}$ is the covariate that affects the observation of the true species and $\xi$ is a zero mean Gaussian Random field. 

The verified data is converted into a binary detection/non-detection of individual species $i= 1, 2, \ldots, S$. For each location $j$, $V_{.j}$ is a ($S \times 1$) matrix with entries:
  \[
    V_{ij} = \left\{\begin{array}{lr}
        1, & \text{if the verified species at location $j$ is species $i$ } \\
        0, & \text{Otherwise } 
        \end{array}\right\}.
  \]
As such, given the mean intensity at location $j$,
\begin{equation}
    V_{.j}|\lambda_{ij} \sim Multinomial (p_{.j});
\end{equation}
where $p_{ij} = \frac{\lambda_{ij}}{\sum_i \lambda_{ij}}$ is the probability of the verified species being species $i$ at location $j$. The verified data could also be seen to be generated from a categorical distribution with probabilities $p_{ij}$, in which case we need not to convert the data into a binary detection/non-detection data.

Assuming the verified species information represents the true point pattern for the species under study, each reported information from the Citizen Scientist was then seen as a draw from any of the $S$ species under study with a given probability. Moreover, we also propose that there is a chance that the true species can be classified as another species that is not in the $S$ species under study. Therefore, the reported species at location $j$, $Y_j$ is a draw from $S+1$ species with probability $\Omega$.\\

Let $\Omega_{ii'}$ be the probability that a single verified species $i \in \{1, \ldots, S \}$ is classified as species $i'$. The probabilities across all the possible species sum to $1.$ This entire confusion matrix can be expressed as:
\begin{equation}
\mathbf{\Omega} = 
 \begin{bmatrix}
\Omega_{11} & \Omega_{11}& \cdots& \Omega_{1S} & 1-\sum_{j=1}^S \Omega_{1j}  \\
\Omega_{21} & \Omega_{22}& \cdots& \Omega_{2S} & 1-\sum_{j=1}^S \Omega_{2j} \\
\vdots & \vdots & \cdots& \vdots & \vdots\\
\Omega_{S1} & \Omega_{S2} & \cdots & \Omega_{SS} & 1-\sum_{j=1}^S \Omega_{Sj}\\
\end{bmatrix}   
\end{equation}
where the rows correspond to the verified species and the columns correspond to the reported species, with the last column corresponding to the case the species is classified as another species outside the $S$ species under study. Given which verified species was present,

\begin{equation}
    Y_j \sim \text{Categorical}(\Omega_{V_j =1, \cdot}),
\end{equation}
where $\Omega_{V_j =1, \cdot}$ refers to the probability of being classified as another species given which verified species was present at location $j$. 

The data streams as used in this framework is summarised in Figure \ref{fig:explanation}. The hierarchical likelihood of the model proposed is given as follows:
\begin{equation*}
    \begin{split}
        \ln \lambda_{ij} &= X`\beta + \xi \\
        p_{ij} &= \frac{\lambda_{ij}}{\sum_i \lambda_{ij}}\\
        V_{.j} & \sim Multinomial(p_{.j})\\
        Y_j & \sim Categorical(\Omega_{V_j =1, \cdot})
    \end{split}
\end{equation*}

 
\begin{figure}[htbp]
    \centering
\includegraphics[scale= 0.35]{Supplementary figures/Plot for model.png}
\caption{Explanation of the various data streams used in the model for two species, Species $1$ and Species $2$. The framework shows the verified species $1$ and $2$ data, their (mis) classification as Species $1$, Species $2$ or another species with the confusion matrix $\Omega$ and the data as can be downloaded from any Citizen Science database.}
    \label{fig:explanation}
\end{figure}

\subsection{Simulation Study}
We performed a simulation study for $S=3$ species. The true intensity of the mean intensity surface were generated for the $S$ species on a continuous square domain with dimensions $50 \times 50$. We define the location $j$ to be the set of all the locations in this domain. The environment covariate $\textbf{x}$ was also generated by defining a continuous gradient from the bottom to the top of the grid, with the values ranging from $0$ to $1$ as shown in Figure \ref{fig:data plot}A). As noted by \cite{simmonds2020more}, this spatial structure was used for the purpose of interpretation of the results. A Matern covariance structure, parameterised by its variance, smoothness ($\nu$) and scale ($\kappa$) was also assumed for the spatial variation in the random field. The variance parameter was chosen as $0.5$ for all the species, scale parameter was chosen as $1.5$ for all the species.

The intercept of the model for the threes species were chosen as $\beta_{01} =2$, $\beta_{02} =0.5$, and $\beta_{03} =3$. The environmental covariate effect for each species was chosen as $\beta_{11}= -1$, $\beta_{12}= 1.5$ and $\beta_{13}= -1$. We generated the true intensity of the verified species by using the 'spatstat' package \citep{baddeley2005spatstat}. The log intensity of the three species are shown in Figure \ref{fig:data plot} B)-D). 
\textbf{I have to look at the sampled sites. Whether to use a grid for the verification.}

\begin{figure}[htbp]
    \centering
\includegraphics[scale= 0.35]{Supplementary figures/cov plus sampling.png}
\caption{Layout of simulated data from the model parameters chosen over a $50 \times 50$ grid showing A)The environmental covariate \textbf{x}, B) - D) the log intensity (log-Lambda) for Species 1 to 3 (S1 -S3) generated from a log-Gaussian process, E) the sampled locations in the grid (S for sampled and NS for non sampled), F) the verified species at the sampled locations; and G) the reported species at the sampled locations.}
    \label{fig:data plot}
\end{figure}

The simulation was repeated 500 times, and for each run the true intensity was simulated using the same parameters as defined above. This was done to ensure that the results analysed would not be due to randomness.

\subsection{Fitting the model}
\subsubsection{Estimating the parameters}
The model was fitted using a Bayesian modelling framework. All the analysis were done using $R$ software  \citep{chambers2008software}.The model was run with the nimble package \citep{de2017programming}. The priors for $\beta_{0i}$ and $\beta_{1i}$ for $i = 1, 2, \cdots, S$ species was chosen from a normal distribution with mean $0$ and standard deviation of $10$, i.e. $ \beta_{0i} \sim N(0, 10^2)$ and $ \beta_{1i} \sim N(0, 10^2)$. We used the intrinsic Conditionally Autoregressive (ICAR) prior for the spatial field $\xi$ \citep{kery2020applied, de2020nimble}. The inputs for the ICAR (weights, adj, num) were obtained from the 'spdep' package \citep{bivand2015package} and the prior for the precision parameter ($\tau$) was from $\text{Gamma}(0.5,0.5)$. The priors of the confusion matrix ($\mathbf{\Omega}$) was chosen from the Dirichlet distribution with parameter alpha, which has a prior of an exponential distribution with mean $1$.

The MCMC was run for $500000$ number of iterations for $5$ chains, and the first $200000$ iterations were chosen as the burn-in. The fitted model was ignored when the model did not converge (looking at traceplots and with gelman statistic value greater than 1.1), showed an error in the running of the model as well as having a small effective sample size. The convergence was done with the 'mcmcOutput' package (\textbf{Check for the citation later}) in $R$. We keep the tenth of the remaining samples in each of the chains. 

With the additional data from the verification, the model is identifiable like any other occupancy and abundance model that also accounts for false positives, even without replicated data \citep{wright2020modelling, chambert2015modeling}.

With the spatially replicated additional data from the verification, the model is identifiable like any other occupancy and abundance model that also accounts for false positives \citep{wright2020modelling, chambert2015modeling}. However, the model should be identifiable when the LGCP is used to model the intensity from a point process. 

\subsubsection{Evaluation of model parameters}
The model parameters $\mathbf{\beta_0}$, $\mathbf{\beta_1}$ and $\mathbf{\Omega}$ were evaluated on a $10 \times 10$ grid (100 locations) by using the mean bias error (MBE). The MBE gives us the average deviation of the estimated parameter value from the truth, with the value to $0$ being better. To assess how well each model fit captured the spatial pattern in each species distribution, the predicted intensity for each species was compared to the true intensity by estimating the correlation between them \citep{simmonds2020more}.

The results were presented with 'ggplot' package \citep{wickham2016package} in $R$ and the codes are attached in the supplementary information.

\subsubsection{Predicting true species abundance}
We also predicted the true species from the estimates of $\mathbf{\Omega}$ to check whether we obtain each true (verified) species intensity and abundance map. With this results, species abundance maps for regions yet to be covered can be predicted from available CS data and the classification probabilities.

Let $\Gamma_{ikj}$ be the probability that the verified species is $i$ given that species $k$ was observed at site $j$. From Bayes theorem,

\begin{equation}
\label{pred true}
    \Gamma_{ikj} = \frac{\text{P(reported = k|verified = i) P(verified=i)}}{\sum_{i}\text{P(reported = k|verified = i) P(verified=i)}}= \frac{\hat \Omega_{ki}\times \frac{\hat \lambda_{ij}}{\sum_i \hat \lambda_{ij}} }{\sum_{i} \bigg [ \hat \Omega_{ki}\times \frac{\hat \lambda_{ij}}{\sum_i \hat \lambda_{ij}} \bigg]},
\end{equation}
for $i = 1,2, \ldots, S$ verified species, $k= 1,2, \ldots ,S+1$ reported species and $j=1,2,\ldots,R$ indexed sites.

The predicted true species was chosen as the species with the maximum of the probability $\Gamma_{ikj}$ for all verified species $i= 1,2, \cdots ,S$. Alternatively, the true species was simulated from Categorical distribution with probability ($\Gamma_{.kj}$) for observed species $k= 1,2, \cdots ,S+1$ at location $j$. Thus, the predicted verified species depends on the estimates of \textbf{$\Omega$} and the predicted mean intensity of each species at the location \textbf{s}.


\subsection{Application to data}

The model was used to analyse Titmouse dataset that was downloaded from iNaturalist, a Citizen Science database \citep{matheson2014inaturalist}. The database hosts over seventy million occurrence observations with well over a million observers. The observers collect these occurence records and upload their observations with images, sounds and other valuable information that can allow for verification \citep{matheson2014inaturalist}. The species name provided by the observer is known as species guess. The observations reported goes through iNaturalist community verification, and is accepted as a research grade when two-thirds of the community agree to the taxon identification \citep{ueda2020inaturalist}. 

We obtained 31901 observations of the titmouse collected over three countries, Canada (358 observations), Mexico (998 observations) and United States (390362 observations). There were five species reported and they were black crested titmouse (\textit{Baeolophus atricristatus}), tufted titmouse (\textit{Baeolophus bicolor}), oak titmouse (\textit{Baeolophus inornatus}), juniper titmouse (\textit{Baeolophus ridgwayi}) and bridled titmouse (\textit{Baeolophus wollweberi}). All other species guess that were not in the comon names listed above were renamed as others. The species guess were used as the reported species and the scientific name (community verifications) was used as the verified species. We also used Ml to classify the data we have and use that as the another alternative for the verified species.

\begin{figure}[htbp]
    \centering
\includegraphics[scale= 0.36]{Supplementary figures/plot of data.png}
\caption{The titmouse dataset downloaded from iNaturalist used for the analysis. The data are facetted according to the scientific name and colored according to the species guess.}
    \label{fig:data}
\end{figure}


 We used the intrinsic Conditionally Autoregressive (ICAR) prior for the spatial field $\xi$ \citep{kery2020applied, de2020nimble}. The inputs for the ICAR (weights, adj, num) were obtained from the 'spdep' package \citep{bivand2015package} and the prior for the precision parameter ($\tau$) was from $\text{Gamma}(0.5,0.5)$.
 
 The data streams as used in this framework is summarised in Figure \ref{fig:explanation}.
\begin{figure}[htbp]
    \centering
\includegraphics[scale= 0.35]{Supplementary figures/Plot for model.png}
\caption{Explanation of the various data streams used in the model for two species, Species $1$ and Species $2$. The framework shows the verified species $1$ and $2$ data, their (mis) classification as categories $1$, category $2$ or category $3$ with the confusion matrix $\Omega$ and the data as can be downloaded from any Citizen Science database.}
    \label{fig:explanation}
\end{figure}

The true intensity of the mean intensity surface were generated for the $S$ species on a continuous square domain with dimensions $50 \times 50$. We define the location $j$ to be the set of all the locations in this domain. The environment covariate $\textbf{x}$ was also generated by defining a continuous gradient from the bottom to the top of the grid, with the values ranging from $0$ to $1$ as shown in Figure \ref{fig:data plot}A). As noted by \cite{simmonds2020more}, this spatial structure was used for the purpose of interpretation of the results. 

The intercept of the model for the threes species were chosen as $\beta_{01} =2$, $\beta_{02} =0.5$, and $\beta_{03} =3$. The environmental covariate effect for each species was chosen as $\beta_{11}= -1$, $\beta_{12}= 1.5$ and $\beta_{13}= -1$. We generated the true intensity of the verified species by using the 'spatstat' package \citep{baddeley2005spatstat}. The log intensity of the three species are shown in Figure \ref{fig:data plot} B)-D). 
\textbf{I have to look at the sampled sites. Whether to use a grid for the verification.}

\begin{figure}[htbp]
    \centering
\includegraphics[scale= 0.35]{Supplementary figures/cov plus sampling.png}
\caption{Layout of simulated data from the model parameters chosen over a $50 \times 50$ grid showing A)The environmental covariate \textbf{x}, B) - D) the log intensity (log-Lambda) for Species 1 to 3 (S1 -S3) generated from a log-Gaussian process, E) the sampled locations in the grid (S for sampled and NS for non sampled), F) the verified species at the sampled locations; and G) the reported species at the sampled locations.}
    \label{fig:data plot}
\end{figure}

\begin{figure}[htbp]
    \centering
\includegraphics[scale= 0.35]{Supplementary figures/predicted true species.png}
\caption{Predicted verified species (VS) using the maximum probability of $\Gamma_{ijk}$ (maxprob) and simulation of the verified species from categorical distribution using $\Gamma_{ijk}$.}
    \label{fig:results2}
\end{figure}


That is, the model reparameterises equation \eqref{intensity} as:

\begin{equation}\label{reparameterised intensity}
     \ln \bigg(\frac{\lambda_{i}}{\lambda_{i'}}\bigg)= (\beta_{0i} - \beta_{0i'}) +  (\beta_{1i} - \beta_{1i'})'\textbf{x} , \quad i \ne i'
\end{equation}
where $\beta_{0i}$ is the intercept of species $i$, $\beta_{1i}$ is the covariate effect and $\textbf{x}$ is the covariate that affects the observation of the verified (true) species for $i=1,2,\ldots, S$ number of species (Proof is attached in the appendix). This is the equation for the multinomial logit model \citep{Fahrmeir2013} and is the exact distribution the verified species were generated from. Moreover, from the equation \eqref{reparameterised intensity}, any of the values of the parameters $\beta_{0i}$ or $\beta_{1i}$ is zero, the estimated value will be unbiased, as is the case for $\beta_{1i}$ in our study. 


\begin{table}[htbp]
    \centering
    \begin{tabular}{p{1.5cm}p{1.5cm}p{2cm}p{3.0cm}p{1.5cm}p{0cm}}
    \hline
\centering Parameter & \centering True value &\centering Median &\centering 95\% CI &\centering Precision &\\ \hline \hline
\centering $\beta_{01}$ &\centering 2 &\centering -0.34 &\centering [-0.47 , -0.14] & \centering 10.11&\\ 
\centering $\beta_{02}$ &\centering 3 &\centering 0.67 &\centering [0.52 , 0.87] & \centering 10.52&\\ 
\centering $\beta_{03}$ &\centering 2 &\centering -0.32 & \centering [-0.49 , -0.15] &\centering 9.77&\\ 
\centering $\beta_{11}$ &\centering  1&\centering 1.01 &\centering [0.84 , 1.20] &\centering 8.88&\\ 
\centering $\beta_{12}$ &\centering  0&\centering 0.01 &\centering [-0.18 , 0.24] & \centering 8.59&\\ 
\centering $\beta_{13}$ &\centering -1 &\centering -0.99 &\centering [-1.18 ,-0.75] & \centering 8.38&\\ \hline
\centering $\Omega_{11}$ &\centering 0.7 &\centering 0.71 &\centering [0.66 , 0.75]  & \centering 45.93&\\ 
\centering $\Omega_{21}$ &\centering 0.15 &\centering 0.16 &\centering [0.13 , 0.17] & \centering 75.09&\\ 
\centering $\Omega_{31}$   &\centering 0.09 &\centering 0.09 &\centering [0.07 , 0.10] &\centering 100.97&\\ 
\centering $\Omega_{12}$   &\centering 0.05&\centering 0.05  &\centering  [0.04 , 0.06]& \centering 112.62&\\
\centering $\Omega_{22}$   &\centering 0.70 &\centering 0.70 &\centering [0.68 , 0.73] &\centering 59.41&\\ 
\centering $\Omega_{32}$   &\centering 0.18  &\centering 0.18 &\centering [0.16 , 0.21] &\centering 62.60&\\ 
\centering $\Omega_{13}$   &\centering  0.13&\centering 0.12  &\centering [0.10 , 0.15] &\centering 75.35&\\
\centering $\Omega_{23}$   &\centering 0.10 &\centering 0.10 &\centering [0.09 , 0.12] &\centering 121.57&\\ 
\centering $\Omega_{33}$   &\centering 0.7 &\centering 0.70 &\centering [0.66 , 0.74] &\centering 55.83&\\ 
\centering $\Omega_{14}$   &\centering 0.12 &\centering 0.12 &\centering [0.10 , 0.15] &\centering 67.91&\\ 
\centering $\Omega_{24}$   &\centering 0.05 &\centering 0.05 &\centering [0.04 , 0.06]  &\centering 146.49&\\ 
\centering $\Omega_{34}$   &\centering 0.03 &\centering 0.03 &\centering [0.03 , 0.06] &\centering 139.54&\\ \hline
    \end{tabular}
    \caption{True values and posterior summaries of estimates of parameters from the simulation study. All the results are converted to two decimal places.}
    \label{reults_simulation}
\end{table}

We modelled the data by using the log-Cox Gaussian point process (LGCP) to account for the spatial dependency in the data. The mean intensity was defined as:

\begin{equation}
 \ln (\lambda_{ij})= \beta_{0i} +  \beta_{1i}  \textbf{$x_1j$} + \beta_{2i}  \textbf{$x_2j$}+\beta_{3i}  \textbf{$x_3j$} + \xi  ,
\end{equation}
where $\beta_{0i}$ is the intercept of species $i$, $\beta_{1i}, \beta_{2i} $ and $\beta_{3i}$ are covariate effect of $x_1$, $x_2$ and $x_3$ respectively which affects the observation of the true species and $\xi$ is a zero mean Gaussian Random field.

The intrinsic Conditionally Autoregressive (ICAR) prior was used for the spatial field $\xi$ \citep{kery2020applied, de2020nimble}. The inputs for the ICAR (weights, adj, num) were obtained from the 'spdep' package \citep{bivand2015package} and the prior for the precision parameter ($\tau$) was from $\text{Gamma}(0.5,0.5)$. The priors of the confusion matrix ($\mathbf{\Omega}$) was chosen from the Dirichlet distribution with parameter alpha, which has a prior of an exponential distribution with mean $1$. The results are presented in Figure \textbf{reference for the figures and tables of the results}.

\begin{figure}[htbp]
    \centering
\includegraphics[scale= 0.075]{Supplementary figures/bias_boxplot.png}
\caption{Boxplot of the bias in contrast of intercept and covariate effect with species $1$ as reference for the 1000 simulated data points. The red vertical  dashed line indicates where the estimates are unbiased.}
    \label{fig:results1}
\end{figure}


\begin{table}[htbp]
    \centering
    \begin{tabular}{p{1.5cm}p{1.5cm}p{1.5cm}p{2cm}p{3.0cm}p{1.5cm}p{0cm}}
    \hline
Species&\centering Category & \centering $\Omega$ &\centering $\hat{\Omega}_{med}$ &\centering 95\% CI &\centering Precision &\\ \hline \hline
\centering $1$ &\centering ${1}$ &\centering 0.7 &\centering 0.69 &\centering [0.61 , 0.78]  & \centering 21.87&\\ 
\centering $2$&\centering  &\centering 0.10 &\centering 0.10 &\centering [0.07 , 0.16] & \centering 44.37&\\ 
\centering $3$&\centering  &\centering 0.00 &\centering 0.00 &\centering [0.00 , 0.00] &\centering $1.2 \times 10^5$&\\ \hline
\centering $1$&\centering ${2}$   &\centering 0.05&\centering 0.05  &\centering  [0.01 , 0.09]& \centering 4.91&\\
\centering $2$&\centering   &\centering 0.80 &\centering 0.79 &\centering [0.74 , 0.85] &\centering 3.14&\\ 
\centering $3$&\centering    &\centering 0.00  &\centering 0.00 &\centering [0.00 , 0.00] &\centering $1.16 \times 10^5$&\\ \hline
\centering $1$&\centering ${3}$   &\centering  0.13&\centering 0.13 &\centering [0.07 , 0.19] &\centering 32.20&\\
\centering $2$&\centering   &\centering 0.05 &\centering 0.05 &\centering [0.03 , 0.09] &\centering 60.23&\\ 
\centering$3$&\centering    &\centering 0.90 &\centering 0.9 &\centering [0.84 , 0.96] &\centering 34.98&\\ \hline
\centering $1$&\centering ${4}$   &\centering 0.12 &\centering 0.12 &\centering [0.08 , 0.18] &\centering 35.39&\\ 
\centering $2$ &\centering   &\centering 0.05 &\centering 0.05 &\centering [0.03 , 0.09]  &\centering 62.62&\\ 
\centering$3$&\centering    &\centering 0.10 &\centering 0.10 &\centering [0.05 , 0.16] &\centering 34.99&\\ \hline
    \end{tabular}
    \caption{True values and posterior summaries of estimates of the classification probabilities from the simulation study. All the results are rounded to two decimal places.}
    \label{reults_omega}
\end{table}


It was also observed that as the temperature increased from February to August 2019, the log intensity for the monarch also increased and the log intensity reduced as the altitude increased within January to June and October to December 2019. This is what we expect since the monarch flies to low lands during the summer, as noted by \cite{zipkin2012tracking}. 


It was also observed that in the months of February to September 2019, the proportion of false positives were for the queen butterfly was very high (the misclassification was higher for the other category). This was because these months saw an increase in the reported species by the Citizen scientists, and as the number of misclassification increased in proportion of the amount of data collected. 

Moreover, the posterior distributions of $\beta_{0i}$ and $\beta_{1i}$ were influenced by the priors used for them. A normal prior with a large standard deviation led to non-convergence, and the model converged only with a strict prior (normal distribution with standard deviation of 1).

The estimates of the parameters $\beta_{0i}$ and $\beta_{1i}$ were biased, because they are not identifiable. However, t

The cases where the estimates has a coverage of approximately $0$ were the instances where the true classification probabilities were $0$. As the model does not estimate the value at exactly $0$ we would not find the true value in all the simulations. This is not a problem, since it would require us very large samples to get a zero as an estimate from the model. 

\section*{Data availability}
All the code, data and supplementary information are available openly on Dyrad with DOI: https://doi.org/10.5061/dryad.37pvmcvmz.

\section*{Acknowledgements}
 This work is part of the NTNU digital transformation project Transforming Citizen Science for Biodiversity.  
 
 \section*{Conflict of Interest}
The authors declare no conflicts of interest.

\section*{Authors Contribution}
KPA, RBA and AF were involved in the conception of the idea for this paper. KPA, RBA, AF and WK were involved in developing of the various parts of this paper and writing of the manuscript. KPA and RBA developed the design for the simulation studies and data application and KPA wrote the code, conducted all analysis and analysed the output.



Attempts at estimating the heterogeneity in 

Common approaches to applying an SDM is to fit single species distribution models (SDMs) (involving the modelling of each species individually) to a taxon or stack the individual SDMs for each taxon for a community \citep{caradima2019individual}. Studies have shown that this stacked SDMs have limitations which includes difficulty in identifying parameters of rare parameters \citep{caradima2019individual, guisan2011sesam}, overpredicting species richness \citep{caradima2019individual, elith2006novel}. Moreover, some species cooccur and show variation in behavioural plasticity when faced with threats \citep{chambert2018two, madsen2020determining}, making management decisions based on single species unreliable \citep{madsen2020determining}.

To alleviate the limitations of the single species distribution models, 

Accounting for  in SDMs have been developing field in recent years. In multi-species literature, one species can be detected or encountered but identified as another species, misidentification \citep{spiers2022estimating}. In this study, we collectively describe these false positives and misidentifications as misclassification. 



The misclassifcation (False positives and negatives) have been treated as homogenuous across various locations, and to our best of knowledge no work has been done on accounting for heterogeneity in misclassification probability. A usual attempt to solving this problem would be to have a seperate model for each observer in the observer-specific classification probability, but in this study a joint model is fit and each observer effect is retrieved from the paramter estimates.

In this study, we propose a general framework that models the heterogeneity in misclassification that allows for inter-taxonomic classifications and predict the true species identity given the observed species identity. The mdodel is parameterized with butterfly data coolected in North America fro 2018 to 2019 which was downloaded from iNaturalist. 

In this study, we assume the verified data is on the individual species-level and the reported classification categories are also on the species level, but include morphospecies \citep{spiers2022estimating}.

\begin{figure}[htbp]
    \centering
\includegraphics[scale= 0.36]{Supplementary figures/butterfly_data_plot.png}
\caption{The subset of the butterfly dataset downloaded from iNaturalist used for the analysis. The data are faceted according to the true species name and coloured according to the reported category.}
    \label{fig:data}
\end{figure}

We subsetted and used the data where an observer has made more than 400 observation between the year 2018 and 2020. The observers whose data were used and the number of observations used are presented in Appendix [\textbf{present that}].

The North American monarch butterfly has an annual multigenerational migration cycle and for every fall, those at the rocky mountains travels long distances to the summer breeding grounds, where most of them aggregate together \citep{culbertsonlong}. \cite{culbertsonlong} noted that climatic changes affects this migration as \cite{zipkin2012tracking} adds that this is a major driver in its population dynamics. Some of these climatic factors are precipitation, temperature and elevation of the area \citep{brym2020prevalence}. Moreover, although the mimicry of the viceroy butterflies somehow depends on the abundance of the queen butterfly \citep{prudic2019mimicry}, these butterflies are co-mimics and have greater resemblance between the patterns \citep{ritland1991revising}, suggesting that the abundance of one of them affects the other in the location. Owing to this information, 



We explored the behaviour and use of this model by analysing both simulated and gull datasets under six scenarios: a) \texttt{covariate} model, b) \texttt{fixed-covariate} model, c) \texttt{fixed-intercov} model, d) \texttt{intercept} model, e) \texttt{constant} model and (f) \texttt{main} model. 

The \texttt{covariate} model fits the MMGLM defined by equation \eqref{linear_predictor_classification} for the classification process by including the covariate that describes the classification process. The \texttt{simplified-covariate} model fits the MMGLM by assuming that the classification covariate $\textbf{z}$ affects only the probability of correctly classifying the states. The \texttt{fixed-intercov} model fits the MMGLM by assuming that the classification covariate $\textbf{z}$ affects only the probability of correctly classifying the states, and the intercept for correctly classifying the states is constant. The \texttt{intercept} model fits the MMGLM for the classification process by ignoring the covariate that describes the classification process and includes an intercept in the MMGLM. The \texttt{constant} models the classification probabilities as generated from Dirichlet distribution with parameter $\alpha$ (this is what is used by \cite{wright2020modelling, spiers2022estimating}); and \texttt{main} model fits the constant model for the classification process but adds the covariate for the classification process to the ecological process model. We presented two different homogeneous models, \texttt{constant} and \texttt{intercept} model, to assess the effect of choosing the Dirichlet prior on the results, as \cite{spiers2022estimating} noted an effect of the prior on the estimates of the classification probability. The specification of the linear predictor for these models is presented in Supplementary information S3.

We model the mean intensity of the reported states as follows:
\begin{equation} \label{ML_intensity}
 \ln (\lambda_{ik})= \beta_{0k} + \sum_{j = 1}^{n_e} x_{ij}\beta_{jk}  ,
\end{equation}
where $\beta_{0k}$ is the intercept of reported state $k$, $\beta_{jk}$ is the effect of covariate $j$ on intensity of reported state $k$, $x_{ij}$ is the $j^{th}$ covariate that affects the observation of the reported state at location $i$ and $n_e$ is the number of covariates in the ecological process model.

We consider $i = 1,2, \ldots, R$ observations, each of which is one of the $s = 1, 2, \ldots, S$ true states (ie. the actual state of observation $i$ is individual $s$). The observations are at location $l_i$. Here we assume that that $l_i \in D \in R^2$, but this assumption can be easily changed, for example, the locations can be in the discrete space. Note that we can allow multiple observations at one location. Using the observation confirmation model (that is, we have access to verified data for some of the states), the sources of data available come from the verified data (labelled as \textbf{V}), which we assume to be the true species identity and reported or classified data (labelled as \textbf{Y}).

These mSDMs can be hierarchical, constraining taxon-specific parameters accounting for overarching community parameters or through the joint SDMs that model the interdependencies between taxa that are jointly inferred \citep{caradima2019individual}.

==> ConflictOfInterest.tex <==
\section{Conflict of Interest}
The authors declare no conflict of interest. 

==> DataAvailability.tex <==
\section{Data Availability}
The Gulls data used for this paper can be downloaded from GBIF (\url{https://doi.org/10.15468/dl.h24bp5}). All codes used for this paper are available at Datadyrad with \url{https://doi.org/10.5061/dryad.0rxwdbs51}.

==> Discussion.tex <==
\section{Discussion}

The main objective of this paper was to propose a general framework to account for misclassifications from imperfect classifications (such as those from surveys) and uncertain classifications (from automated classifiers) in mSDMs. This work builds on previous work by \cite{spiers2022estimating, wright2020modelling} by accounting for the heterogeneity in the classification probabilities while allowing the classified categories to be more than the verified species (such as unknown species, morphospecies etc.). Moreover, we assessed the effect of overfitting a homogeneous classification process on the predictive performance of mSDMs and provided ways of checking the overfitting of the classification process model. 

Our study bridges the knowledge gap in the literature on accounting for misclassification in mSDMs by modelling the heterogeneity in the classification process. False positives are inevitable in biodiversity data \citep{miller2013determining, kery2020applied}. To model these false positives in this study, we presented the true state observation process as one model and the classification process as another model in a hierarchical form. We model the classification probabilities for each true state identity as a multinomial generalised linear model. This specification generalises the modelling of the classification process to model effects of covariates as fixed or random effects or both. For example, one can estimate the classification probabilities of each observer in volunteer-collected data by assuming a random observer effect. This formulation for the classification process also mitigates the modelling problems of using the Dirichlet distribution as the prior for the classification probabilities  \citep{spiers2022estimating}.

Furthermore, the specification of a separate state-space model for the true state observation process in the proposed framework allows the use of various multi-species observation models (such as joint species distribution models \citep{tobler2019joint, ovaskainen_abrego_2020}, Royle-Nichols model for abundance \citep{royle2003estimating}, amongst many others) to model the distribution of the true states. Our simulation study showed that the proposed model framework could estimate the true state relative abundance parameters (with the bias of estimated parameters close to zero; Supplementary information 2; S2-1), an observation noted in previous studies that use observation confirmation design to model misclassification in mSDMs \citep{spiers2022estimating, wright2020modelling, kery2020applied}. We have shown that the true state observation process model is a simplified form of occupancy and abundance models that account for misclassification (Table \ref{tab:generalisation}), so we believe our proposed framework can be extended to any design used to collect and verify data on the true states (for example, point processes, distance sampling, site-confirmation (multi-method) design, etc.), and any model used to fit the data (for example, multi-state occupancy model \citep{kery2020applied}, joint species distribution models \citep{tobler2019joint,ovaskainen_abrego_2020}).

Modelling the true state observation process with more complex models than the relative abundance models used in the study would add another level of hierarchical structure to the true state observation process (for example modelling detection probability or true occupancy state). This complexity could introduce confounding of the classification process and observation process parameters and with frequentist estimation approaches make the likelihood multi-modal \citep{kery2020applied}. This study did not explore such issues and further work can be done on this. A possible solution in the Bayesian framework to avoid such confounding issues would be to model the different processes with separate covariates, choose a good prior for the mSDM parameters, and use repeated survey visit data to model the true state observation process \citep{kery2020applied}. Moreover, the identifiability or confounding issues could also be tackled by using data with much information on detection and false positive detections such as those derived from acoustic surveys \citep{clement2022estimating} and integrating occupancy data that are not susceptible to misclassifications such as those from camera traps to those with misclassifications \citep{kery2020applied}.

Accounting for the heterogeneity in the classification process increases the predictive performance of mSDMs. The homogeneous classification models may sometimes be unable to explain the variation in the classification process \citep{conn2013accommodating}, leading to poor model predictive performance \citep{montesinos2022overfitting}. The simulation study showed a 30\% increase in precision and a 6\% decrease in accuracy and recall when the heterogeneity in the classification process was accounted for in the mSDMs (Figure \ref{fig:accuracy_and_precision} A, B). However, there was no change in predictive performance when a heterogeneous classification model overfitted a homogeneous classification process (Figure \ref{fig:accuracy_and_precision} A, B) due to the small classification covariate effect size, observed from the bias of parameter estimates and low Bayesian variable selection probability (Figure \ref{fig:accuracy_and_precision} A, B). Since the predicted posterior probability for the true state's identity heavily relies on the weights from the misclassification probability (Supplementary Information 1), failure to account for that would mean our posterior probability would be incorrectly estimated. The incorrectly predicted probability would lead to the underestimation of the prediction of the ranges of coverage and possibly abundance in the true states \citep{molinari2012monitoring}.

Fitting a more complex true state observation model with the covariate that explains the heterogeneity of the classification process does not provide enough information to improve the mSDM's predictive performance. Previous studies have shown that the estimates of the observation process model inform the estimation of the classification probabilities \citep{spiers2022estimating}, but the variability in the classification process cannot be inferred from variability in the observation process model (Figure \ref{fig:accuracy_and_precision} A (i - iii), Supplementary Information 1). Ecologists should therefore model the variability in the classification in its process model to gain the advantage in the mSDMs predictive performance.

Our model was parameterised with volunteer-collected gull data. These volunteer-collected data have several sources of bias in their generation, such as spatial bias, and misidentification of species, among many others. We acknowledge that all these sources of biases may be present in the data, but we only modelled the misidentification of species by using the number of previously collected data as a proxy measure for the observer's experience in the classification process model. The predictive performance of the homogeneous and heterogeneous models was approximately the same due to small misclassified samples (19 misclassified out of 1382 samples in training data (Supplementary Information S2-2) and 10 misclassified out of 378 samples in validation data (Supplementary Information S2-3)). However, the estimated covariate effect gives an idea of how the experience affects the probability of classifying a new observation. Specifically, the probability of correctly identifying the correct species increases with the observer's experience, as is noted in some literature \citep{santos2021understanding, vohland2021science, johnston2018estimates, kelling2015can}. Therefore, there is a trade-off between the model's ability to correctly classify mismatched data (precision) and understanding the covariate's effect driving the classification process when there are relatively small misclassified samples. 

The inclusion of ML prediction scores in the mSDMs to account for the heterogeneity in the classification process increased the precision of our predictions by 70\% (Table \ref{tab:data_validation}). These ML prediction scores are observation specific and provide much information about the classification process to increase the precision of the model. The information from the ML does not depend on the misclassified sample sizes but on the quality of the images \citep{koch2022maximizing}, making them advantageous to use in accounting for heterogeneity in the classification process when misclassified sample sizes are small (like we have in our gull data). 

The proposed model framework in this study is flexible and can be generalised into any species distribution model and integrated distribution model. The framework proposed fits into the frameworks provided by \cite{wright2020modelling} and \cite{spiers2022estimating} and any framework their study generalises. Our proposed classification process model, MMGLM, improved the predictive performance of mSDMs, but it heavily relies on the misclassified samples size. Furthermore, the confusion matrix defined in the model framework allows for the classification of different taxonomic groups, as opposed to just the species by species confusion matrix in \cite{wright2020modelling} and including morphospecies in the classification categories \citep{spiers2022estimating}. This will make it possible for citizen science data analysts to account for the misclassification of data at any level in the data collection process. We recommend that variable or model selection is performed during the analysis to check for overfitting. Moreover, ecologists should explore using ML prediction scores (where the prediction scores are available) as weights in mSDMs that aim at predicting true state distributions especially when the data has a small misclassified sample size.




==> Methodology.tex <==
\nopagebreak
\section{Methodology}
\label{section:methodology}

\subsection{Model framework}
The proposed framework assumes a model for where the true state's identity is "present" (we use "state(s)" in this work to refer to taxon identity as well as any other identification category or morpho-states, such as an unidentified group). This true state can be on any taxonomic level. However, the true states are often unknown and treated as latent. An individual is sampled and classified as another state, known as the "reported" or "classified" state, with a probability. These reported states can also be on any taxonomic level or any unidentified group \citep[such as in studies that include morphospecies;][]{spiers2022estimating}. We further assume that the individuals are verifiable (and that we have information on the verification process) and that the verified state approximates the true state identity. 

\subsubsection{True state observation process model}

We specify a relative abundance model (specifically a multinomial logit model) for the true state observation process. Our objective is to show how to model heterogeneity in the classification process and not to make inferences about the true state's abundance, so we chose a model that was easier to fit and understand to explain the distribution of the true state.  

Let $\lambda_{is}$ be the average number of $s = 1,2,\ldots, S$ true individuals  at location $i =1,2,\ldots, R$, which describes the abundance of the true states over space.  This means that intensity can be modelled as an inhomogeneous point process (PPM) which assumes that the data are dependent on the environment covariate, or as a log-Cox Gaussian Point process (LGCP) where we assume a spatial dependency in the observed data \citep{renner2015point}. Here, the mean intensity is modelled using the inhomogeneous  point process and defined as:

\begin{equation} \label{intensity}
 \ln (\lambda_{is})= \beta_{0s} + \sum_{j = 1}^{n_e} x_{ij}\beta_{js}  ,
\end{equation}
where $\mathbf{\beta_{0s}}$ is the intercept of state $s$, $\beta_{js}$ is the effect of covariate $j$ on the intensity of true state $s$, $x_{ij}$ is the $j^{th}$ covariate that affects the observation of the state at location $i$ and $n_e$ is the number of covariates in the observation process model. Note that we assume there are no species interactions in our relative abundance model, and this could have been added as a random effect in the true state intensity definition (equation \eqref{intensity}).

Let $p_{is}$ be the probability of true state $s$ being at location $i$. We estimate this probability from the mean intensities as follows:

\begin{equation}\label{proportion}
    p_{is} = \frac{\lambda_{is}}{\sum_{s}\lambda_{is}},
\end{equation}
where $\lambda_{is}$ is given by \eqref{intensity}. 

The true state $s = 1,2,\ldots, S$ at location $i=1,2,\ldots, R$ is then a realisation from a categorical distribution with probability $p_{is}$. 

This model specification for the ecological process used here is similar to the occupancy dynamics and encounter rate model used by \cite{spiers2022estimating} by assuming that occupancy probability equals one; and similar to the model used by \cite{wright2020modelling} by assuming Poisson counts with intensity $\lambda_{is}$ (refer to Table \ref{tab:generalisation} for the link between our model framework and that of \cite{spiers2022estimating} and \cite{wright2020modelling}.).

\subsubsection{Classification process model}
For each observation, we assume there was imperfect classification and that the true state identities can be classified into $k = 1, 2, \ldots, K$ states. Assuming the true state distribution represents the true point pattern for the species under study, each reported information can be seen as a draw from any of the $K$ states under consideration with a given probability. As mentioned above, these states could be on any taxonomic level or include any unidentified group. For example, one could have four true states: common gull, herring gull, Audouin's gull and Sooty gull. These species can be reported in three states: large while-headed gulls, large black-headed gulls and other gulls. An example of the classification probability (confusion matrix) is shown in Table \ref{example}. 

\begin{table}[ht!]
\centering
\begin{tabular}{||c| c c c||} 
\hline
& & \textbf{Reported states} & \\

 \textbf{True states} & Large white-headed gulls & Large black-headed gulls & Other gulls \\ [0.5ex] 
 \hline\hline
Common gull & 0.8 & 0.1 & 0.1 \\ 
Herring gull & 0.9 & 0 & 0.1 \\
Audouin's gull & 0 & 0.9 & 0.1 \\
Sooty gull & 0 & 1 & 0 \\ [1ex] 
 \hline
\end{tabular}
\caption{Example of confusion matrix that applies to our model.}
\label{example}
\end{table}

 Let $\Omega_{sk}$ be the probability that a single true state $s \in \{1, \ldots, S \}$ is classified as state $k \in \{1, \ldots, K \}$. The probabilities across all the possible $k$ states sum to $1$. In studies with homogeneous classification probabilities, the confusion matrix for the classification can be expressed as:
\begin{equation}\label{omega_matrix}
\mathbf{\Omega} =  \begin{bmatrix}
\mathbf{\Omega}_{1}   \\
\mathbf{\Omega}_{2}  \\
\vdots \\
\mathbf{\Omega}_{S}  \\
\end{bmatrix}  =
 \begin{bmatrix}
\Omega_{11} & \Omega_{11}& \cdots & \Omega_{1k}& \cdots& \Omega_{1K}   \\
\Omega_{21} & \Omega_{22}& \cdots& \Omega_{2k}& \cdots& \Omega_{2K} \\
\vdots & \vdots & \cdots& \vdots & \cdots& \vdots\\
\Omega_{S1} & \Omega_{S2} & \cdots & \Omega_{Sk}& \cdots& \Omega_{SK} \\
\end{bmatrix}   
\end{equation}
where the rows correspond to the true states $s$ and the columns correspond to the reported states $k$. 

We model the heterogeneity in the classification probabilities by fitting a multinomial generalised linear model \citep{Fahrmeir2013} to each of the rows of $\mathbf{\Omega}$ defined in equation \eqref{omega_matrix}. We refer to this approach as the multiple multinomial generalised linear model (MMGLM, hereafter). We define the linear predictor of the MMGLM as:
\begin{equation}\label{linear_predictor_classification}
\begin{split}
\zeta_{isk} &= \omega_{0sk}+ \sum_{j = 1}^{n_c} z_{ij}\omega_{jsk}\\
&= 
 \begin{bmatrix}
{\omega_0}_{11} & {\omega_0}_{12}&  \cdots& {\omega_0}_{1K}   \\
{\omega_0}_{21} & {\omega_0}_{22}&  \cdots& {\omega_0}_{2K} \\
\vdots & \vdots & \cdots& \vdots\\
{\omega_0}_{S1} & {\omega_0}_{S2} & \cdots& {\omega_0}_{SK} \\
\end{bmatrix}   + \ldots + \begin{bmatrix}
{\omega_n}_{11} & {\omega_n}_{12}&  \cdots& {\omega_n}_{1K}   \\
{\omega_n}_{21} & {\omega_n}_{22}& \cdots& {\omega_n}_{2K} \\
\vdots & \vdots &  \cdots& \vdots\\
{\omega_n}_{S1} & {\omega_n}_{S2} &  \cdots& {\omega_n}_{SK} \\
\end{bmatrix}* z_{in_c}  \\
\text{and in matrix notation:}\\
\boldsymbol{\zeta}_i & = \boldsymbol{\omega_0} + \sum_{j = 1}^{n_c}\boldsymbol{\omega_j} z_{ij} ;
\end{split}
\end{equation}
 where $\boldsymbol{\omega_{0}}$ is an $S \times K$ matrix of intercepts and $\boldsymbol{\omega_{j}}$ is an $S \times K$ matrix of covariate $j$ effects, and $z_{ij}$ is the $j^{th}$ covariate that drives the classification process at location $i$. Using equation \eqref{linear_predictor_classification} as the definition for the linear predictor, our estimates of the parameters $\omega_{0sk}$ and $\omega_{jsk}$ are identifiable with reference to one reported state. Therefore for each true state identity $s$, the classification probabilities for each reported state $k=1, 2, \ldots, K-1$ with reference to state $K$ is modelled as:
\begin{equation}\label{heterogenous}
    \ln \bigg(\frac{\Omega_{sk}}{\Omega_{sK}}\bigg) = ({\omega_0}_{sk} - {\omega_0}_{sK}) + ({\omega_1}_{sk} - {\omega_1}_{sK})*\textbf{z}_{1} + \ldots +({\omega_n}_{sk} - {\omega_n}_{sK})*\textbf{z}_{n};
\end{equation}
where $\textbf{z}_{1}$, $\ldots$, $\textbf{z}_{n}$ are covariate vectors.

This general framework has $S \times (K-1) \times (n_c +1)$ parameters to be estimated, where $S$ is the number of true states, $K$ is the number of reported states, and $n_c$ is the number of covariates in the classification process. Estimating these parameters can be very computationally expensive as the number of true states, reported states and covariates increases and would require significant numbers of misclassified state samples to estimate them. Therefore, we explored simplified forms of the generalised model in equation \eqref{heterogenous}.

A simplified case of equation \eqref{heterogenous} assumes that the classification covariate \textbf{z} only affects the probability of correctly classifying the states. In this instance, the matrix $\boldsymbol{\omega_j}$ has its off-principal diagonal elements $\omega_{jsk} = 0$ for $s \neq k$ for covariate $j$, and these parameters are not estimated (This is our study scenario "fixed-covariate" in Table \ref{tab:scenarios}). This simplification reduces the number of parameters estimated for the classification process by $n_c \times (K - S - 1)$, where $S$ is the number of true states, $K$ is the number of reported states and $n_c$ is the number of classification covariates. A further simplification would also assume that the average probability of correctly classifying the true state does not change with species, that is, $\omega_{0sk}$ is the same for all $s = k$ (This is our study scenario "fixed-intercov" in Table \ref{tab:scenarios}). The classification process heterogeneity is captured by the covariate effect $\omega_{1sk}$ for all $s=k$. The latter further reduces the number of parameters estimated by $S - 1$. This last simplification is useful especially when the states are very similar, and one would expect that their average classification probabilities would be the same.

Given which true state ($s$) was present at location $i$, the reported state at that location is a draw from $K$ states with probability $\mathbf{\Omega}$.
\begin{equation}
    Y_i|V_{i} = s \sim \text{Categorical}(\Omega_{is \cdot}),
\end{equation}
where $\Omega_{is.}$ refers to the probability of being classified as any of the $K$ states given that the true state identity at location $i$ is state $s$.

\subsubsection{Variable selection}
Fitting a complex model with these many parameters can result in an overfitted model. An overfitted model captures the pattern and noise in the training data, but performs poorly on validation or test data \citep{montesinos2022overfitting}. In some cases, the true state observation and classification process covariates may be highly correlated. These correlated covariates can inflate standard errors (reduce the precision) of the estimated parameters \citep{yu2015multicollinearity, roberts2017cross, caradima2019individual}. To avoid overfitting the model, there is a need to perform variable selection. In this study, we performed Bayesian variable selection, specifically the spike and slab prior to the classification process covariates \citep[for review of Bayesian variable selection see][]{o2009review}. For each of the classification process covariates, we re-define the linear predictor in equation \eqref{linear_predictor_classification} as:

\begin{equation} \label{variable selection}
\begin{split}
    \zeta_{isk} &= \omega_{0sk}+ \sum_{j = 1}^{n_c} \psi_{j}z_{ij}\omega_{jsk};\\
    \text{with} \quad \psi_{j} &\sim Bernoulli(q_j)
\end{split}
\end{equation}
where $\psi_{j}$ is the indicator that variable $j$ is selected with the expected probability $q_j$. The variable selection indicator specified in equation \eqref{variable selection} jointly selects the variable that affects all the true states in the model but can also be made state-specific \citep{ovaskainen_abrego_2020}. Probabilities $q_j$ closer to $1$ indicate that the variable contributes much to the model and should be selected, and those closer to $0$ indicate that the variable contributes less and can be discarded.  

\begin{table}[htbp!]
%
\tablestyle[sansbold]
%
\begin{tabular}{|p{0.16\linewidth}|p{0.15\linewidth}|p{0.3\linewidth}|p{0.39\linewidth}|}
\theadstart
  \thead Classification type &\thead Model & \thead True state observation process & \thead Classification process \\

\tbody
 %
   Heterogeneous   & Variable / covariate & $\ln(\lambda_{is}) = \beta_{0s} + x_{1i}\beta_{1s}+ x_{2i}\beta_{2s}$ & $\ln(\frac{\zeta_{isk}}{\zeta_{isK}}) = \omega_{0sk} + \psi_{i} z_{1i}\omega_{1sk}$ \\ \hline
         & fixed-covariate & $\ln(\lambda_{is}) = \beta_{0s} + x_{1i}\beta_{1s}+ x_{2i}\beta_{2s}$ & $\ln(\frac{\zeta_{isk}}{\zeta_{isK}}) = \omega_{0sk} + \psi_{i} z_{1i}\omega_{1ss}$, \par $\text{where $\omega_{1sk} = 0 $ for $s \ne k$}$  \\ \hline
         & fixed-intercov & $\ln(\lambda_{is}) = \beta_{0s} + x_{1i}\beta_{1s}+ x_{2i}\beta_{2s}$ & $\ln(\frac{\zeta_{isk}}{\zeta_{isK}}) = \omega_{0sk} + \psi_{i} z_{1i}\omega_{1ss}$, \par $\text{where $\omega_{1sk} = 0$ for $s \ne k$}$ \par $\text{and $\omega_{0sk}$ is the same for $s=k$}$  \\ \hline
   Homogeneous      & intercept & $\ln(\lambda_{is}) = \beta_{0s} + x_{1i}\beta_{1s}+ x_{2i}\beta_{2s}$ & $\ln(\frac{\zeta_{isk}}{\zeta_{isK}}) = \omega_{0sk}$ \\ \hline
        &  constant & $\ln(\lambda_{is}) = \beta_{0s} + x_{1i}\beta_{1s}+ x_{2i}\beta_{2s}$ & $\Omega_{sk} \sim Dirichlet(\alpha_{sk})$,\par $\text{where $\alpha_{sk} \sim Exp(1)$}$ \\ \hline
         & main & $\ln(\lambda_{is}) = \beta_{0s} + x_{1i}\beta_{1s} + x_{2i}\beta_{2s} + \psi_{i} z_{1i}\beta_{3s}$ & $\Omega_{sk} \sim Dirichlet(\alpha_{sk})$, \par $\text{where $\alpha_{sk} \sim Exp(1)$}$  \\ \hline
 %
 %\tsubheadstart
 %\tsubhead subhead &
% \tsubhead subhead \\
 %
 %content  & content \\
 %content  & content \\
 \tend
\end{tabular}
\caption{Variations in the MMGLM for the classification process defined by equation \eqref{variable selection} and observation process defined by equation \eqref{intensity} used as our study scenarios. There are three heterogeneous models: covariate, fixed-covariate and fixed-intercov, and three homogeneous models: intercept, constant, and main. }
\label{tab:scenarios}
\end{table}

\subsection{Modelling heterogeneity using ML prediction scores}
Some studies give weight to the true identities of the reported observations or state, for example, because they use machine learning to classify the observation. These prediction scores (such as $F_1$ score, mean square error, and logarithmic loss) are not  classification probabilities but are values that indicate how well the ML algorithm classifies data in the test sample. We can use this information to model the heterogeneity in the classification process and predict the true state identity as follows:

\begin{equation} \label{MLAlgorithm}
\begin{split}
 V_i| Y_i &\sim \text{Categorical} (p_{iks}); \\ 
 \text{with} \quad p_{iks} &= \frac{\lambda_{ik}w_{iks}}{\sum_{k} \lambda_{ik}w_{iks}}
\end{split}
\end{equation}
where $\lambda_{ik}$ is the average abundance of reported state $k$ at site $i$ and $w_{iks}$ is the predictive score of the $k^{th}$ reported state to true state $s$ at sampling unit $i$. 

It must be noted that this approach is a non-parametric approach to account for heterogeneity in the classification whereas the MMGLM is a parametric approach. Moreover, modelling the heterogeneity in the classification process using ML prediction scores models the covariate effects on the expected abundance of the reported states and corrects them using the prediction scores as weights to obtain the relative abundance of the true states. However, the MMGLM models the covariate effect on the expected abundance of true states and estimates the heterogeneity in the classification process using a parametric model. The prediction of the true state identity is done by weighing the expected intensity of true states with the estimated classification covariate.

\subsection{Generalisation of model framework}
The proposed framework generalises the existing mSDMs that account for misclassification in occupancy models. \cite{wright2020modelling} provided a framework to account for the homogeneity in the classification process, and our model is connected to this by using the relationship between the multinomial and the Poisson distribution \citep{steel1953relation} for the observation process as well as using a species by species constant model for the classification process (Table \ref{tab:generalisation}). \cite{wright2020modelling} further provided arguments that their proposed models were generalised forms of models for the binary detection of two species \citep{chambert2018two}, single species with count detections \citep{chambert2015modeling} and single species with binary detections \citep{chambert2018new}. Since our proposed framework can be seen as  a heterogeneous version of \cite{wright2020modelling}, our framework is also a generalisable form of the models in \cite{chambert2015modeling, chambert2018new, chambert2018two}. \cite{spiers2022estimating} provided an individual-level semi-supervised approach that estimates species misclassification with occupancy dynamics and encounter rates, and our model is connected to this if we assume a homogeneous classification process (that is $\boldsymbol{\omega_1} = \textbf{0}$), and assume that the occupancy probability is $1$ (Table \ref{tab:generalisation}).

\begin{table}[htbp!]
\tablestyle[sansbold]
%
\begin{tabular}{|p{0.2\linewidth}|p{0.4\linewidth}|p{0.4\linewidth}|}
\theadstart
\thead \centering Author &
\thead \centering Model Framework&
\thead \centering Link to our model \tabularnewline
\tbody
%
\cite{wright2020modelling} and the models their proposed framework generalises such as \cite{chambert2015modeling, chambert2018new, chambert2018two} &
\textit{True state observation process: absolute counts}

$z_{is} \sim \text{Bernoulli}(\psi_{is})$

$[V_{ijs}| z_{is} = 1] \sim \text{Poisson}(\lambda_{ijs})$
 &
\textit{True state observation process: relative abundance}

Choose $\psi_{is} = 1$, then $z_{is} = 1$ for all locations $i$ and true states $s$.

 $[V_{ijs}| z_{is} = 1] \sim \text{Poisson}(\lambda_{ijs})$ using the relationship between multinomial and Poisson distribution \citep{steel1953relation}.
 \\
&
\textit{Classification process:}

$[Y_{ijs}|V_{ijs} = v_{ijs}, z_{is} = 1 ] \sim \text{Multinomial}(v_{ijs}, \Omega_{sk})$, 

where $\Omega_{sk} \sim \text{Dirichlet}(\alpha)$ &
 

\textit{Classification process:}

$[Y_{ijs}|V_{ijs} = 1, z_{is} = 1 ] \sim \text{Categorical}(\Omega_{sk})$, 

where $\Omega_{sk}$ can be chosen as any of the homogeneous models described in Table \ref{tab:scenarios} \\ \hline

\multirow{ 2}{*}{\cite{spiers2022estimating}} &
\textit{True state observation process: occupancy dynamics and encounter rates}

     $z_{ist} \sim \text{Bernoulli}(\psi_{ist})$

$[V_{ijst}]  \sim Categorical \bigg(\frac{\lambda_{ijst}z_{ist}}{\sum_s \lambda_{ijst}z_{ist}} \bigg)$;
&
\textit{True state observation process: relative abundance}

 Choose $ t = 1, \psi_{ist} = 1$, then $z_{ist} = 1$ for all locations $i$ and true states $s$. 

$[V_{ijs}] \sim Categorical \bigg(\frac{\lambda_{ijs}}{\sum_s \lambda_{ijs}} \bigg)$;

\\
&
\textit{Classification process:}

$[Y_{ijs}|V_{ijs}] \sim \text{Categorical}(\Omega_{sk})$, 

where $\Omega_{sk} \sim \text{Dirichlet}(\alpha)$ &
 

\textit{Classification process:}

$[Y_{ijs}|V_{ijs} = 1] \sim \text{Categorical}(\Omega_{sk})$, 

where $\Omega_{sk}$ can be chosen as any of the homogeneous models described in Table \ref{tab:scenarios}.


\\
\tend
\end{tabular}
\caption{Extensions of our proposed models from homogeneous classification process studies done by \cite{wright2020modelling} and \cite{spiers2022estimating}. The table specifies the true state observation process model for \citeauthor{wright2020modelling} (absolute abundance model), \citeauthor{spiers2022estimating} (occupancy dynamics and encounter rate model) and ours (relative abundance model); and also the classification process model for \citeauthor{wright2020modelling} and \citeauthor{spiers2022estimating} (homogeneous classification process with classification probabilities simulated from Dirichlet distribution) and ours from heterogeneous models described in Table \ref{tab:scenarios}. Since our framework extends the work done by \citep{wright2020modelling}, it is safe to say that they are also generalised forms of \cite{chambert2015modeling, chambert2018new, chambert2018two}.  }
\label{tab:generalisation}
\end{table}

\subsection{Simulation Study} \label{simulation study}
\label{subsection:simulation study}
To demonstrate how our proposed model works and its use in prediction, we performed a simulation study for $S=2$ true states, and $K=3$ reported states over $R=1000$ sites. We simulated two covariates for the true state observation process and one for the classification, all from a Normal distribution with a mean of $0$ and variance of $1$. The true intensity was simulated from equation \eqref{intensity}. The intercepts of the model for the two true states were chosen as $\beta_{01} = -1$, $\beta_{02} = 0$ and covariate effect for each true state was chosen as $\beta_{11}= 4$, $\beta_{12}= -2$, $\beta_{21}= 0$ and $\beta_{22}= 0$ (that is, state $2$ is used as a reference category). The intercept and covariate effect for the classification process was chosen as follows:
\begin{equation*}\label{values}
\begin{split}
\omega_{0}&= 
 \begin{bmatrix}
2 & 0.5 & 0   \\
1 & 1 & 0 \\
\end{bmatrix}; \omega_{1} =\begin{bmatrix}
3 & -1 &   0   \\
-1 & 1 & 0 \\
\end{bmatrix}.
\end{split}
\end{equation*}

These values were chosen to obtain significant sample sizes of misclassified states. We simulated $200$ datasets with a heterogeneous classification process using the variable model in Table \ref{tab:scenarios} (referred to as the "\textbf{full model}"), $200$ with a homogeneous classification process by assuming $\boldsymbol{\omega_{1}} = \textbf{0}$ (a matrix of zeros) in equation \eqref{heterogenous} (referred to as "\textbf{reduced model}") and another $200$ with the covariate effect for the classification process (using the variable model in Table \ref{tab:scenarios}) that is correlated to the true state observation process covariate  (referred to as "\textbf{correlation model}"). The first simulated dataset explored modelling heterogeneity's effect on the classification process, whereas the latter explored the effect of having correlated covariates for the classification and true state observation process. The second assessed the effect of overfitting the classification process model (adding heterogeneity to the classification process when it should be homogeneous). Moreover, we assessed the impact of the number of misclassified samples on the mSDMs predictive performance. We increased the principal diagonal components of $\boldsymbol{\omega_{0}}$ by $6$ to obtain a reduction in the number of misclassified samples simulated.

We randomly withheld two hundred of the true state identities for each dataset simulated as our validation sample. The number of validation samples was not varied since \cite{spiers2022estimating} found that the number of validation samples had a modest effect on the model's predictive ability. We fitted the model under the various scenarios described in Table \ref{tab:scenarios} to the data and evaluated the model's predictive performance on the validation sample. 

\subsection{Case study: Gulls dataset} \label{case study}
The proposed model was used to analyse gull dataset downloaded from GBIF (\cite{gbif}). The database hosts over two billion occurrence observations with well over a million observers (website visited on 17th February 2023). We were interested in the iNaturalist records since they have community verifications \citep{matheson2014inaturalist}. The observers collected these occurrence records and uploaded their observations with images and/or sounds that allowed for verification.  The reported observations go through iNaturalist community verification and are accepted as research grade when two-thirds of the community agreed to the taxon identification \citep{ueda2020inaturalist}, at which point they are published on GBIF. We assumed that the community-accepted taxon name is the true state \textbf{V}. We checked the iNaturalist platform to track the identification process of the observations and use the first reported identification as the reported state \textbf{Y}.

We obtained observations for some species of gulls in Denmark, Finland and Norway from 2015 to 2022. Specifically, we selected great black-backed gulls (\textit{Larus marinus}), herring (\textit{Larus argentatus}), common gulls (\textit{Larus canus}) and lesser black-backed gulls (\textit{Larus fuscus}) because the iNaturalist website reported that these species are commonly misclassified as the other. Any other species reported apart from the above-mentioned species were labelled as "others". We used annual precipitation \citep[accessed from the raster package; ][]{hijmans2015package} as true state observation process covariates in the model since it has been noted in some literature to affect the distribution of sea birds such as gulls \citep{jongbloed2016flight, algimantas2010abundance}.

The data obtained were presence-only records. Exploratory analysis revealed that there were no multiple observations at the same location for our selected species. We, therefore, assumed that our locations were discrete and treated the data as a marked point process, where the species that was reported at a location is given a value of $1$ and $0$ for the other species in this study. If we had a species list, then we could have modelled it as a repeated marked point process at the same location and treated the sites as a random effect.

Citizen science data are known to be affected by several sources of bias. Some common biases are spatial bias \citep{johnston2022outstanding, tang2021modeling}, and misclassifications \citep{johnston2022outstanding, tulloch2013realising}. We only accounted for the misclassifications in this study, as we are interested in explaining the classification process and not making inferences about the abundance of the gulls. Citizen scientists have been reportedly known to correctly classify species as they gain experience reporting the species \citep{vohland2021science}. We, therefore, modelled the variation in the classification process by using the number of reports made by each observer as a covariate in the classification process. If an observer has more than ten observations, the extra number of observations was calibrated at $10$. We used this number of observations for an observer as a measure of experience \citep{johnston2018estimates, kelling2015can}, although there are other indices for measuring effort or experience of the citizen scientist \citep{santos2021understanding, vohland2021science}. 

We also used ML algorithm to obtain prediction scores (specifically $F_1$ scores) for the possible true state identity of our downloaded data. The ML algorithm was a Convolutional Neural Network \citep[a modified form in ][]{koch2022maximizing} trained with data from all citizen science observations of any species in Norway. Since the ML algorithm is trained with all birds data from GBIF in Norway, we trained all our six study scenarios models summarised in Table \ref{tab:scenarios} with all data for our selected gull species in Norway and all data reported before 2022 in Finland and Denmark and used all data reported in 2022 in Finland and Denmark as our validation sample. The summary of the classifications (true and false positives) in the training and validation sample is presented in Supplementary information 2 (S2-2, S2-3).

\subsection{Fitting and evaluating the model}
%\subsubsection{Estimating the parameters}
We ran all the analyses using the Bayesian framework using the Markov chain Monte Carlo approach in the NIMBLE package \citep{de2017programming} using the R software \citep{Rsoftware}. We chose the priors for all true state observation parameters from a normal distribution with a mean of $0$ and standard deviation of $10$, and we chose the priors for the classification process parameters from Normal distribution with a mean of $0$ and standard deviation of $1$. For the scenarios: constant and main model, we chose the priors of the confusion matrix ($\Omega$) from the Dirichlet distribution with parameter alpha ($\alpha$), which has a prior of an exponential distribution with mean $1$.

We ran 3 chains, each with 10000 iterations; the first 5000 iterations were chosen as the burn-in. We check the convergence of the models by visually inspecting the trace plots and ignoring models with a Gelman-Rubin statistic \citep{brooks1998general} value greater than $1.1$. We kept a fifth of the remaining samples in each of the chains.

We used accuracy (the proportion of predicted true states identities from all the predictions of the validation samples), precision (the proportion of mismatched true states in the validation sample that were correctly classified from the predictions) and recall (the proportion of correct true states in the validation sample retrieved from the predictions) as performance metrics. We used a Bayesian approach and got the posterior distributions for the parameters. Higher values of the validation metrics indicated the preferred model. We also checked how well the model estimated the true state observation process parameters ($\boldsymbol{\beta_0}$, $\boldsymbol{\beta_1}$ and $\boldsymbol{\beta_2}$) and the classification process parameters ($\boldsymbol{\omega_0}$ and $\boldsymbol{\omega_1}$) by estimating the bias (difference between the true value and the estimated value) and precision of the parameters. 

==> Results.tex <==
\nopagebreak
\section{Results}

\subsection{Simulation study}

%Figure \ref{fig:bias in parameters} presents the bias in the estimates of the parameters from the simulation study and figure \ref{fig:accuracy_and_precision} presents the accuracy and precision of the six simulation models under study. 

\subsubsection{Predictive performance}

 We illustrated the gain in model performance by using the accuracy, recall and precision of our model's predictions (Figure \ref{fig:accuracy_and_precision} A and B). When data was simulated from the full and correlated models, there was a strong indication that the predictive performance of mSDMs improved when the variability in the classification process was included. That is the "variable" model performed best for the full and correlation models with the highest accuracy, recall and precision values (Figure \ref{fig:accuracy_and_precision} A (i - ii), B (i - ii)). The simplified heterogeneous models (fixed-intercov and fixed-covariate) however did not perform any better than the homogeneous models (Figure \ref{fig:accuracy_and_precision} A (i - ii), B (i - ii)). This suggested that simplifying the heterogeneous classification model did not yield any improvement in predictive performance, and the heterogeneous model that captures the entire variability (in this case variable model; Table \ref{tab:scenarios}) would be the best predictive model. When the classification process covariate was modelled as part of the observation process (main model), the model's predictive performance also performed similarly to the homogeneous models (Figure \ref{fig:accuracy_and_precision} A and B). 
 
 \begin{figure}[ht!]
    \centering
\includegraphics{Figures/metrics.png}
\caption{Boxplot of validation metrics (accuracy, precision, recall) from the six study models defined in Table \ref{tab:scenarios} on the two hundred (200) withheld samples out of the thousand (1000) samples simulated in each dataset. Accuracy is the proportion of withheld samples that were correctly classified, recall is the proportion of correctly classified samples that were retrieved from the withheld samples, and precision is the proportion of the misclassified samples that were correctly classified. Each boxplot shows the median and the interquartile range (25 - 75\% quartiles). Each column shows the type of model used to simulate the dataset: "full" refers to using the variable/covariate model  in Table \ref{tab:scenarios}, "reduced" refers to using the intercept model in Table \ref{tab:scenarios} and "correlation" refers to using the variable model in Table \ref{tab:scenarios}, but with correlated true state observation and classification process covariates. The rows correspond to changes made to the number of misclassified samples in the simulated dataset: "Baseline" refers to using the values defined in section \ref{simulation study} and "Decrease" refers to reducing the number of misclassified samples by diagonal elements of $\mathbf{\omega}$ by 6 as described in section \ref{simulation study}}
    \label{fig:accuracy_and_precision}
\end{figure}

 Overfitting a homogeneous classification process with a heterogenous one did not have any effect on the mSDM's predictive performance (Figure \ref{fig:accuracy_and_precision} A iii) and B iii)). We expected the overfitted heterogeneous models to have poor predictive performance \citep{montesinos2022overfitting}, but the heterogeneous and homogeneous performed similarly (with equal recall, accuracy and precision across all six study models). The Bayesian variable selection probability indicated that the homogeneous classification model was better (with the probability of including classification covariates in heterogeneous models being $0.359 \pm 0.012$; Supplementary information 2; S2-1). Although the simplified heterogeneous models did not yield improvement in predictive performance, they performed similarly to the variable model in the variable selection process.

\subsubsection{Effect of number of misclassified samples}
As we increased the number of misclassified samples in our simulated data, the precision increased by on average $30 \%$ and accuracy and recall reduced by $6 \%$ (Figure \ref{fig:accuracy_and_precision} A (i - ii), B (i - ii)). This decrease in accuracy and recall could be attributed to the reduction in the number of correct classifications in the simulated data as the number of misclassified samples increased. Moreover, the classification parameters were estimated better when the number of misclassified samples was higher, leading to the high precision of predictions (Supplementary information 2; S2-1). This suggested that our proposed model will be beneficial when one has a substantial number of misclassified samples.

\subsubsection{Bias in observation and classification process parameters}
 Although failure to account for misclassification in mSDMs can result in biased true state observation process parameters \citep{wright2020modelling, spiers2022estimating}, any method used to account for misclassification in mSDMs has a small effect on the accuracy and precision of the true state observation process parameters. The bias of the observation process parameters was consistently low for all six models, and the coverage was higher for all the scenarios under the full and reduced model (Supplementary information 2; S2-1). All the scenarios studied accounted for misclassification of some sort, thereby correcting for the bias in the observation parameters estimates \citep{wright2020modelling, spiers2022estimating}. The classification process parameters were estimated more accurately and precisely for the variable model than the other models (Supplementary information; S2-1). This was only possible in the case where we had enough misclassified samples. This suggests that if the objective of a study is to predict true state identity with mSDMs, then modelling the full heterogeneity can improve predictive performance; if the aim is inference on true state distribution, then heterogeneous models may not provide any advantage over homogeneous models. 

\begin{table}[htbp!]
%
\tablestyle[sansbold]
%
\begin{tabular}{*{5}{p{0.18\textwidth}}}
\theadstart
   \thead Method & \thead Accuracy & \thead Precision & \thead Recall & \thead Variable selection probability\\

\tbody
 %
        Variable / Covariate & 0.97 & 0.1 & 0.99 & 0.71\\ \hline
        Constant & 0.97 & 0.1 & 0.99 & - \\ \hline
        Intercept & 0.97 & 0.1 & 0.99 & -\\ \hline
        Main & 0.97 & 0.1 & 0.99 & 0.29 \\ \hline
        Fixed intercov & 0.97 & 0.1 & 0.99 & 0.70\\ \hline
        Fixed covariate & 0.97 & 0.1 & 0.99 & 0.71 \\ \hline
        Machine Learning & 0.89 & 0.8 & 0.90 & - \\ \hline
 %
 %\tsubheadstart
 %\tsubhead subhead &
% \tsubhead subhead \\
 %
 %content  & content \\
 %content  & content \\
 \tend
\end{tabular}
\caption{Validation metrics of the models under study on the withheld gull dataset. The accuracy is the proportion of correctly classified validated data, the precision is the proportion of mismatched identities that were correctly matched and recall is the proportion of correctly matched identities that were recovered. The number of validated samples was 384 out of which 10 were mismatched.}
\label{tab:data_validation}
\end{table} 

\subsection{Case study: Gull dataset}

All six study scenario models performed equally well regarding their predictive performance with high accuracy and recall but smaller precision (Table \ref{tab:data_validation}). The poor precision value could not be attributed to the insignificance of the classification covariate (observer experience) in explaining the heterogeneity in the classification process since the variable selection probabilities are closer to $1$ (Table \ref{tab:data_validation}) but to the small misclassification sample sizes (Supplementary Information 1; S2-2, S2-3).  However, the precision increased from 10\% to 80\% when the heterogeneity in the classification process was accounted for by using the prediction scores from the Machine learning algorithm (Table \ref{tab:data_validation}). The ML algorithm's prediction scores were individual observation-specific which provided direct information to the observation process model. However, the six classification models depended on the misclassified sample size to capture the heterogeneity in the classification process. This suggests that one remedy to improve mSDM's predictive performance for data with very small misclassified samples is to use ML weights to account for heterogeneity in mSDMs.

\begin{figure}[htbp!]
    \centering
\includegraphics{Figures/classifyProbs.png}
\caption{Summary of results from the model fit to gull dataset showing A) Probability of correct classification for the common (\textit{Larus canus}), herring (\textit{Larus argentatus}), great black-backed (\textit{Larus marinus}) and lesser black-backed gulls (\textit{Larus fuscus}) and B) the distribution of the experiences of the observers used in the modelling. The ribbon around the correct classification probability estimates represents the 95 \% credible interval of the estimates.}
    \label{fig:omega}
\end{figure}

Although the study scenario models had smaller precision, it was observed that the probability of correctly classifying the gull species in Denmark, Finland and Norway increased with the experience of the observer (Figure \ref{fig:omega}). The pattern showed that observers have a high chance of making mistakes on their first few reports, and they get better as the number of reports increased \citep{vohland2021science}. 



==> Supplementary1.tex <==
%\section{Supplementary Information Two for 'Accounting for Misclassification in Multispecies distribution models'.}
\section{Supplementary information 1}

\textbf{Equivalent Representation of Equation (1) and (2) to the multinomial logit model}.

We want to show that the model definition for the verified species in the main text can be easily modified to the multinomial logit model. Given the data with $c= 1,2,\ldots, C+1$ categories, \cite{Fahrmeir2013} defined the multinomial logit model as described below

\begin{equation} \label{multinomial logit}
    log(\frac{\pi_c}{\pi_{C+1}}) = X'\beta,
\end{equation}
where $\pi_c$ is the probability of observing category $c$, $\pi_{C+1}$ is the probability of observing reference category $C+1$, $\beta$ is a vector of coefficients and $X$ is the design matrix.

Let us define $s'$ as the reference species, for $s' \in \{1,2,\ldots, S\}$. Given the intensity for the species $s$ as defined by equation (1), then the proportion of having verified species $s$ as defined by equation (2) becomes:

\begin{equation}
    \begin{split}
        p_{is} = P(\text{verified species} = s)= \frac{e^{\beta_{0s} + \beta_{1s} x_i}}{\sum_s e^{\beta_{0s} + \beta_{1s} x_i}}
    \end{split}
\end{equation}

The ratio of the proportion of observing verified species $s$ relative to the reference verified species $s'$ at site $i$ becomes:
\begin{equation}
    \begin{split}
        \frac{p_{is}}{p_{is'}} &= \frac{e^{\beta_{0s} + \beta_{1s} x_i}}{e^{\beta_{0s'} + \beta_{1s'} x_i}}\\
        \implies log \bigg(\frac{p_{is}}{p_{is'}} \bigg) &= (\beta_{0s} - \beta_{0s'}) + (\beta_{1s} - \beta_{1s'})x_i\\
        &= X'\beta
    \end{split}
    \label{mylogit}
\end{equation}
which is the same as the multinomial logit model defined in equation \eqref{multinomial logit}.


==> Supplementary2.tex <==
\section{Supplementary Information 2}
\subsection*{Model Representation as a general form of misclassification in multispecies SDMs.}

Our proposed model in the main text is a generalisation of the model framework proposed by \cite{wright2020modelling} which provides a general framework for modelling misclassification in multispecies distribution models. We first present our model into the model framework described by \cite{wright2020modelling} and then by the deductions made in their paper, establish the generalisations of our framework. Since \cite{spiers2022estimating} is an extension of the work by \citep{wright2020modelling}, their work fits into our model framework.

\subsection*{a. Model Framework by \cite{wright2020modelling}.}

Let $z_j$ be the true presence/absence state for site $j$. Then $z_j \sim \text{Bernoulli}(\psi_j)$, where $\psi_j$ is the occupancy probability. Let $Y_{ij}$ be the latent detection counts for each species $i$ at site $j$, that is, $Y_{ij} \sim \text{Poisson} (\lambda_i)$ and the observed counts given the latent detection counts $[C|Y=y] \sim \text{Multinomial}(y, \Theta)$, where C and $\Theta$ are K-length vectors and $\Theta$ is the confusion matrix.

The joint distribution of C and Y is then:
\begin{equation*}
    \begin{split}
        P(C=c,Y=y) &= Pr(C=c|y=y) P(Y=y)\\
        &= \bigg[\frac{1}{c_1!} (\lambda \theta_1)^{c_1}e^{-\lambda \theta_1}\bigg] \bigg[\frac{1}{c_2!} (\lambda \theta_2)^{c_2}e^{-\lambda \theta_2}\bigg] \cdots \bigg[\frac{1}{c_k!} (\lambda \theta_k)^{c_k}e^{-\lambda \theta_k}\bigg]
    \end{split}
\end{equation*}
and as such the probability mass function for each $c_k$ is that of a Poisson distribution with rate parameter $\lambda \theta_k$. Hence $[C_{ik.k'}|Z_i] \sim \text{Poisson} (\sum_{k=1}^K z_{ik} \lambda_{ij} \theta_{kk'})$, where $z_i$ is the vector of occupancy at site $i$ for all $K$ species used in their studies.



\subsection*{b) Connection between our framework and that of \cite{wright2020modelling}.}
The deductions made by \cite{wright2020modelling} hangs on the proof that the marginal distribution of the observed species counts being Poisson. We therefore show that the distribution of the observed counts (reported category) are Poisson distributed, and as well all the deductions by \citep{wright2020modelling} holds. 

The hierarchical likelihood of the model in the main article was:
\begin{equation*}
    \begin{split}
        \ln (\lambda_{is}) &= \textbf{x}'\beta \\
        p_{is} &= \frac{\lambda_{is}}{\sum_i \lambda_{is}}\\
                Y_{i} &\sim Poisson (\Lambda = \sum_{s=1}^S \lambda_{is}) \\
        V_{i} | Y_{i} & \sim Categorical(p_{i.})\\
        \textbf{C}_i | {V}_{i}& \sim categorical(\Omega_{V_i, \cdot})
    \end{split}
\end{equation*}
where $\textbf{C}$ denotes the reported or observed category, $\textbf{V}$ denotes the verified state and ${Y}$ denotes the total number of verified states for site $i$ for $s= 1, \ldots, S$ verified states, $k=1,2,\ldots, K$ reported categories and $i=1, 2, \ldots,R$ number of sites. It must be noted that the categorical distribution used in the main article is the multinomial distribution with $Y=1$ for all the sites, since we assumed that we can only observe one state at a site. In that case, 

\begin{equation}
    P(Y=1) = \Lambda e^{-\Lambda}
\end{equation}

The joint distribution of $\textbf{V}$ and $Y$ is:
\begin{equation}
\begin{split}
    P(\textbf{V}=\textbf{v}, Y=1) &= \bigg[ \  p_1 ^{v_1}p_2 ^{v_2} \cdots p_s ^{v_s}\bigg] \bigg[ \Lambda^y e^{-\Lambda}\bigg] \\
    &= \bigg[ (\Lambda p_{1})^{v_1} e^{-\Lambda p_{1}}\bigg]\bigg[  (\Lambda p_{2})^{v_2} e^{-\Lambda p_{2}}\bigg] \cdots\bigg[(\Lambda p_{s})^{v_s} e^{-\Lambda p_{s}}\bigg] 
    \end{split}
\end{equation}
This implies that the marginal distribution of each verified state $V_s$ is a Poisson distribution with rate parameter $\Lambda p_s$. 

We then proceed to find the marginal distribution of the reported counts $C_k$ for each category given the verified state $v_s$,:
\begin{equation}
    \begin{split}
   P(\textbf{C}=\textbf{c}, V_s= 1) &= P(\textbf{C}=\textbf{c}| V_s= 1)P(V_s= 1)\\
   &= \Omega_{s1}^{c_1}\Omega_{s2}^{c_2} \cdots \Omega_{sK}^{c_K} (\Lambda p_s)e^{\Lambda p_s}\\
   &=\prod_k (\Lambda p_s \Omega_{sk})^{c_k}e^{-\Lambda p_s\Omega_{sk}}
    \end{split}
\end{equation}
where $\Omega_{sk}$ is the sth row and kth column of the confusion matrix $\Omega$ in equation (3) of the main paper. This equation shows that the marginal distribution of the observed or reported counts $C_k$ are Poisson distributed with rate parameter $\Lambda p_s\Omega_{sk}$.

Our result is similar to that of \cite{wright2020modelling}, with the rate parameter of our proposed model scaled by the probability of the verified state $p_s$.

\subsection*{c) Extensions to the other models.}

With the discussions above, we can state that our model is also a generalisation of the two species with binary detection \citep{chambert2018two}, single species with count detections \citep{chambert2015modeling} and single species with binary detections \citep{chambert2018new} with the proof explained by \cite{wright2020modelling}. It can also be extended for other non-occupancy models as explained by \cite{wright2020modelling}.

==> Supplementary_information1.tex <==
\section{Supplementary Information One (S1) for 'Modelling heterogeneity in classification process in multi-species distribution models improves predictive performance.'}

\textbf{Equivalent Representation of Equation (1) and (2)}.

We want to show that the model definition for the verified species in the main text is the multinomial logit model. Given the data with $c= 1,2,\ldots, C+1$ categories, \cite{Fahrmeir2013} defined the multinomial logit model as described below

\begin{equation} \label{multinomial logit}
    log(\frac{\pi_c}{\pi_{C+1}}) = X'\beta,
\end{equation}
where $\pi_c$ is the probability of observing category $c$, $\pi_{C+1}$ is the probability of observing reference category $C+1$, $\beta$ is a vector of coefficients and $X$ is the design matrix.

Let us define $i'$ as the reference species, for $i' \in \{1,2,\ldots, S\}$. Given the intensity for the species $i$ as defined by equation \eqref{intensity}, then the proportion of having verified species $i$ as defined by equation \eqref{proportion} becomes:

\begin{equation}
    \begin{split}
        p_{ij} = P(\text{verified species} = i)= \frac{e^{\beta_{0i} + \beta_{1i} x_j}}{\sum_i e^{\beta_{0i} + \beta_{1i} x_j}}
    \end{split}
\end{equation}

The ratio of the proportion of observing verified species $i$ relative to the reference verified species $i'$ at site $j$ becomes:
\begin{equation}
    \begin{split}
        \frac{p_{ij}}{p_{i'j}} &= \frac{e^{\beta_{0i} + \beta_{1i} x_j}}{e^{\beta_{0i'} + \beta_{1i'} x_j}}\\
        \implies log \bigg(\frac{p_{ij}}{p_{i'j}} \bigg) &= (\beta_{0i} - \beta_{0i'}) + (\beta_{1i} - \beta_{1i'})x_j\\
        &= X'\beta
    \end{split}
\end{equation}
which is the same as the multinomial logit model defined in equation \eqref{multinomial logit}.



==> introduction.tex <==
\section{Introduction}
Species distribution models are essential ecology and conservation management tools that predict how natural and human factors affect biodiversity \citep{elith2009species,vermeiren2020integrating}. With an  increasing amount of biodiversity data from multi-species surveys available to scientists, multi-species distribution models (hereafter mSDMs) have become widely used in analysing these data. These mSDMs  model data at the community level, identify the important variables that drive species co-occurrences and predict the distribution of species in a community \citep{ovaskainen2011making, pollock2014understanding, hui2015multi}. 

However, the biodiversity data obtained from these surveys can be subject to observation errors. These observation errors include false positives (recording absent species as present and misidentifying one species for another) and false negatives (failing to record present species). These false positives are usually a species that has been misclassified. It would be a great advantage if the observation was correctly classified, rather than being discarded once it has been identified as a false positive. The false positives may arise from imperfect classifiers  \citep{wright2020modelling, spiers2022estimating}, observer error, and many other sources. In this study, we collectively describe all the false positives and misidentifications as misclassification and use true states (we use true states to mean the correct identification of the observation) to describe the correct or actual observation identity we are interested in modelling. False negatives are mostly accounted for in occupancy models by modelling the imperfect detection in the observation model. Failure to account for or correct these errors leads to biases in inferences about state variables such as occupancy probabilities, covariate effects and relative activity \citep{ ferguson2015occupancy, wright2020modelling, clare2021generalized}, leading to an impairment in decision making \citep{hoekman2021multi}. 

The methods to deal with misclassification from biodiversity data can be grouped into data review methods and model-based methods \citep{clare2021generalized}. Data review methods require complete and proper data collection and processing methods. This process can be very demanding as it is challenging to control for misclassification. This makes the model-based methods more popular when working with large-scale datasets from large-scale biodiversity data vendors like GBIF \citep{gbif}. Model-based methods estimate classification probabilities jointly with the true state variables of interest. Model-based methods attempting to account for misclassification in multispecies occupancy models currently include modelling misclassification with detection heterogeneity \citep{ferguson2015occupancy, louvrier2018accounting,clement2022estimating}, integrating multiple observers records with other methods such as distance sampling and  N-Mixture models \citep{hoekman2021multi}, supervised methods with extra information from observation confirmation or verification \citep{ferguson2015occupancy, guillera2017dealing}, site confirmation \citep{clare2021generalized} and other calibrated methods. These methods need extra data from the verification process, which helps in estimating the misclassification probabilities in a semi-supervised setting \citep{spiers2022estimating} and makes the parameters in the model identifiable \citep{guillera2017dealing}. The above-mentioned studies have either used verified data collected on the site-level \citep[where the occupancy state of a species is known at a site and not at the individual sample level,][]{chambert2018new}, on aggregated individual sample level using a multinomial model with site-covariates \citep{wright2020modelling}, or on individual sample-level validation data which helps in modelling non-species identities (morphospecies) to species identities \citep{spiers2022estimating}. It is also worth stating that some studies have explored misclassification in abundance \citep{conn2013accommodating} and capture-recapture \citep{augustine2020spatial} models.

Furthermore, these previous studies assumed that the misclassification probabilities are homogeneous (constant) across the study. In reality, the classification probabilities may vary with environmental covariates \citep[such as field conditions;][]{conn2013accommodating} or observer experience \citep[especially when ascertaining how well each observer classifies a report in citizen science projects will be informative;][]{ arazy2021framework, johnston2022outstanding}, distance from a transect when using transect data \citep{conn2013accommodating}, picture quality, etc. An attempt at modelling the heterogeneity in the classification process would be to model this effect as part of the true state model (such as abundance or occupancy). However, this approach may not solve the problem of heterogeneity in the classification process since the estimates of the true state observation process parameters only serve as informed priors to the classification process \citep{spiers2022estimating}. 

A more correct approach to model this heterogeneity is adding the covariate effect to the classification process. Some studies on dynamic false positive single-species occupancy models have modelled temporal changes in false positives using year as a covariate \citep{sutherland2013accounting, miller2013determining, kery2020applied}, showing the possibility to model misclassification trends over time. Our study attempts to model variation in classification probabilities in mSDMs by modelling the probability of classifying a true state identity with a multinomial generalised linear model. To our knowledge, no previous work has been done on this. Failure to account for the heterogeneity in the misclassification probabilities will lead to biased estimates in the parameters of the true state observation process (such as species abundance, richness, and occupancy probabilities) and reduce the model's predictive performance. 

Moreover, recent efforts to correctly classify observations from biodiversity surveys have relied on machine learning (hereafter ML) algorithms  \citep{suzuki2022deep, saoud2020miss, lotfian2021partnership, willi2019identifying,keshavan2019combining, borowiec2022deep, koch2022maximizing}. These ML algorithms use sounds and/or images of observations to predict the true identity of the individual observations, and they can be trained to mimic expert verification of observations \citep{keshavan2019combining, ponti2022human, langenkamper2019impact}. These ML algorithms use a prediction score (a value that shows the weight of predicting the observations as something else) to predict the possible list of the true identities of the individual reported observations. These prediction scores and a list of possible true identities provide information about the classification process of each observation. They can be used to model heterogeneity in the classification process. This study is the first to model the heterogeneity in the classification process by using the prediction scores to weigh the distribution of the reported observations and predict the distribution of the actual observation identities. 

Here, we present a joint model that simultaneously models the true state variables of interest (such as occupancy and abundance) and the heterogeneity in the classification process. Our model set-up extends the work done by \cite{wright2020modelling} and \cite{spiers2022estimating} by a) allowing the classification probabilities to vary with a covariate, b) allowing additional morphostates designations in imperfect classifications (for example, having "unidentified woodpecker" as part of the classified observations), c) using ML prediction scores as weights to account for heterogeneity in the classification process and d) performing variable selection on the classification process covariate to check for potential mSDM overfit. We compared the classification performance of our model with models that assume a homogeneous classification probability done by \cite{wright2020modelling} and \citep{spiers2022estimating} through simulation studies. We parameterise our model  with citizen science data on gulls in Norway, Finland and Denmark from iNaturalist \citep{matheson2014inaturalist} downloaded from the Global Biodiversity Information Facility \citep[GBIF hereafter;][]{gbif}. 

==> rejected.tex <==
Understanding the natural world through various monitoring programmes has become an essential part of ecological conservation, leading to increased knowledge of the ecosystem \citep{ruiz2016uncertainty, jones2011monitoring}. An essential contribution to this goal is the development in the field of Citizen Science (where citizens are involved in data collection and other scientific procedures). Regardless of the benefits in obtaining wider coverage of data to estimate relevant ecological parameters, misclassification remains a critical issue to consider when analysing species distribution models (hereafter noted as SDMs) \citep{bird2014statistical}.

The problem of misclassification has been construed as problems of false positives and false negatives, which are two common sources of biases in Citizen Science data. False positives occur when non-targeted species are reported as the species of interest \citep{clare2021generalized}; and false negatives occur when targeted species are reported as non-targeted species. Many approaches have been developed to account for these false positives and negatives in species distribution models \citep{kery2020applied, wright2020modelling, chambert2015modeling,royle2006generalized}. Out of these, very few are from multi-species distribution models \citep{wright2020modelling,chambert2018two}. There have been increasing literature that supports the assertion that accounting for false positives in single species models are not adequate, especially in instances where the target species can be easily classified as some other species or co-occur with other species \citep{wright2020modelling}. Failure to account for the false positives lead to underestimation of species ranges and biases in estimates of species occurrence or abundance \citep{molinari2012monitoring}. These false positives are actually another individual that has been identified, so it is a misclassification. This work focuses on a general framework for these issues.


The method needs data with both an observation and some validation. These validations can be from Machine learning algorithms (such as \textbf{cite Wouter's app}) or by human expects (such as community verification for iNaturalist data \citep{matheson2014inaturalist}). Although the developments in the ML has led to improvements in classification of individuals reported \citep{willi2019identifying,keshavan2019combining,saoud2020miss}, they do not however provide uncertainty in the estimates of the classification probabilities. We however view the classifications as a verified data and use our method to account for the mis-classification. The additional verified data  makes the estimation of the mis-classification probabilities identifiable like any other occupancy or abundance model \citep{chambert2015modeling, wright2020modelling}.

There are instances where individuals are identified to the genus level or a different level (for example unidentified woodpecker), and this has not been considered in the 
existing model frameworks that account for misclassification in SDMs.  The model framework we propose provides a flexible and general framework that allows inter-taxonomic misclassification such as species - genus classification to be accounted for. 

Another interesting question that has been asked by most ecologists is whether the verified species information can be predicted once the citizen scientist has reported the information. Our model framework makes it possible to continually update the information of the verified species by taking into account the estimated classification probabilities from the available verified information. This can help in the identification of individuals, for example, if an individual is mis-identified as being well out if its range.

The point of this paper is to present a multi-species distribution in two parts: the mis-classification with uncertainties around them and another that estimates the parameters in the model. This model we propose is very flexible and general in its application. The rest of this paper is outlined as follows: the proposed model framework with simulation study and application to data set is presented in section two, the results are presented in section $3$ and the discussions in section $4$.

==> supplementary3.tex <==
\section{supplementary 4}


\begin{sidewaystable}
\setlength\tabcolsep{2pt} % default is '6pt'
\setlength\extrarowheight{2pt}
\caption{Trabalhos Selecionados após critérios de Seleção} 
\label{tab:laal} 
\begin{tabularx}{\textwidth}{|*{16}{C|}}
\hline
Identificador &
Autores & 
Ano & 
Titulo &
Resumo & 
Benefícios & 
Limitações & 
Padrão de Projeto & 
Elementos\slash Padrões Arquiteturais & 
Tecnologias (frame\-works, APIs) & 
Modelo de Acessibilidade & 
Nível Acessibilidade & 
Tipo de Deficiência & 
Tecnologia Assistiva & 
Linguagens & 
Tipo de Avaliação \\ 
\hline
\end{tabularx}

\end{sidewaystable}







\begin{table}[ht!]
%
\tablestyle[sansbold]
%
\begin{tabular}{*{8}{p{0.1\textwidth}}}
\theadstart
        experience & "truth" & Queen & Monarch & Viceroy & other & other danaus & other limenitis \\ 
        \tbody
        
        \hline
        1 & Queen & 4442 & 0 & 0 & 0 & 0 & 0 \\ \hline
        1 & Monarch & 86 & 6780 & 9 & 127 & 1 & 0 \\ \hline
        1 & Viceroy & 2 & 3 & 619 & 2 & 1 & 0 \\ \hline
        2 & Queen & 944 & 0 & 0 & 0 & 0 & 0 \\ \hline
        2 & Monarch & 19 & 1624 & 6 & 18 & 0 & 0 \\ \hline
        2 & Viceroy & 1 & 2 & 201 & 1 & 0 & 2 \\ \hline
        3 & Queen & 687 & 0 & 0 & 0 & 0 & 0 \\ \hline
        3 & Monarch & 10 & 921 & 3 & 30 & 0 & 0 \\ \hline
        3 & Viceroy & 0 & 1 & 90 & 0 & 0 & 1 \\ \hline
        4 & Queen & 110 & 0 & 0 & 0 & 0 & 0 \\ \hline
        4 & Monarch & 3 & 196 & 0 & 79 & 0 & 0 \\ \hline
        4 & Viceroy & 0 & 0 & 13 & 0 & 0 & 0 \\ \hline
        5 & Queen & 18 & 0 & 0 & 0 & 0 & 0 \\ \hline
        5 & Monarch & 3 & 272 & 0 & 3 & 0 & 0 \\ \hline
        6 & Queen & 384 & 0 & 0 & 0 & 0 & 0 \\ \hline
        6 & Monarch & 2 & 600 & 1 & 38 & 0 & 0 \\ \hline
        6 & Viceroy & 0 & 0 & 102 & 0 & 0 & 0 \\ \hline
 \tend
\end{tabular}
    \caption{Crosstabulation of the verified states and reported categories for the training set of the butterfly dataset. The training set was used in fitting the model, and the experience level was used as a covariate in the classification process.}
    \label{training data}
\end{table}

\begin{table}[ht!]
%
\tablestyle[sansbold]
%
\begin{tabular}{*{8}{p{0.1\textwidth}}}
\theadstart
        experience & "truth" & Queen & Monarch & Viceroy & other & other danaus & other limenitis \\ 
        \tbody
        
        \hline
      1 & queen & 1792 & 0 & 0 & 0 & 0 & 0 \\ \hline
        1 & Monarch & 12 & 4080 & 1 & 56 & 1 & 0 \\ \hline
        1 & Viceroy & 0 & 3 & 150 & 0 & 0 & 0 \\ \hline
        2 & queen & 192 & 0 & 0 & 0 & 0 & 0 \\ \hline
        2 & Monarch & 3 & 570 & 0 & 3 & 1 & 0 \\ \hline
        2 & Viceroy & 0 & 0 & 16 & 0 & 0 & 0 \\ \hline
        3 & queen & 202 & 0 & 0 & 0 & 0 & 0 \\ \hline
        3 & Monarch & 1 & 430 & 0 & 0 & 0 & 0 \\ \hline
        3 & Viceroy & 0 & 0 & 12 & 0 & 0 & 0 \\ \hline
        4 & queen & 118 & 0 & 0 & 0 & 0 & 0 \\ \hline
        4 & Monarch & 0 & 113 & 0 & 0 & 0 & 0 \\ \hline
        4 & Viceroy & 0 & 0 & 4 & 0 & 0 & 0 \\ \hline
        5 & queen & 5 & 0 & 0 & 0 & 0 & 0 \\ \hline
        5 & Monarch & 0 & 156 & 0 & 0 & 0 & 0 \\ \hline
        6 & queen & 137 & 0 & 0 & 0 & 0 & 0 \\ \hline
        6 & Monarch & 0 & 272 & 0 & 0 & 0 & 0 \\ \hline
        6 & Viceroy & 0 & 0 & 19 & 0 & 0 & 0 \\ \hline
 \tend
\end{tabular}
    \caption{Crosstabulation of the verified states and reported categories for the validation set of the butterfly dataset. The validation set was used in assessing the predictive performance of the model, and the experience level was used as a covariate in the classification process.}
    \label{tab:validation_data}
\end{table}




==> transferToMainThesis.tex <==
Variable and model selection would be an essential development of this method. This study used a joint spike and slap prior to the classification process variable selection. The number of parameters in the classification process increases exponentially with the number of species, number of classified categories and the number of covariates (number of parameters in the classification process $=$ number of species $\times$ number of classified categories $\times$ number of covariates). This number of parameters requires substantial misclassified samples to correctly estimate the number of parameters in the classification process and model the heterogeneity in the classification process. Obtaining such a sample size would be very challenging for most studies since citizen science projects are currently taking time to orient the observers properly \citep{vohland2021science, johnston2018estimates, kelling2015can}. Further work can explore the state-specific variable selection, ecological and classification process variable selection, and other Bayesian model and variable selection techniques such as WAIC, adaptive shrinkage and model space approaches (Refer to \cite{o2009review} for a review of the variable selection methods). 

==> write_up_rejected.tex <==
\section{Introduction}
Species observations obtained from Citizen Science programs where non-professionals are involved in data collection and other scientific procedures is rapidly becoming an essential part of the knowledge base for ecological conservation. Data collected by these hobbyists has led to a massive increase in the coverage and amount of data collected. This data gives insight into population trends, changes in ranges,  relative abundance, survival and phenological traits of interest in space and time \citep{dickinson2010citizen, bonney2009citizen}.

Citizen science data have several potential challenges such as spatial bias arising from preferential sampling by the citizen scientists \citep{johnston2022outstanding,tang2021modeling, sicacha2021accounting}, errors from identification \citep{gardiner2012lessons,johnston2022outstanding}, among many others. In this paper, we focus on the errors from identification. The errors from identification has been classified as problems of false positives and false negatives. False positives occur when non-targeted species are reported as the species of interest \citep{clare2021generalized}; and false negatives occur when targeted species are reported as non-targeted species or a species is not observed. In this paper, we treat them collectively as misclassification (or misidentification), since both the false positive and negative are misclassified species. Failure to account for the misclassification errors lead to underestimation of species ranges and biases in estimates of species occurrence or abundance \citep{molinari2012monitoring,cruickshank2019quantifying,pillay2014accounting}.

Many approaches have been developed to account for these false positives and negatives in species distribution models \citep{kery2020applied, wright2020modelling, chambert2015modeling,royle2006generalized}. There has been increasing literature that supports the assertion that accounting for false positives in single species models are not adequate, for example when the species co-occur \citep{chambert2018two,wright2020modelling}. This holds especially in instances where the target species can be easily classified as some other species or co-occur with other species \citep{wright2020modelling}. Some attempts have been made to account for these misclassifications in multi-species distribution models \citep{wright2020modelling,chambert2018two}. These approaches use some confirmatory information from the expert, community or automated verifications \citep{chambert2015modeling, chambert2018two, baker2021verification} to explicitly model the misclassification. To our best of knowledge, there is no model that predicts the true species distribution by taking into account the estimates of the classification probabilities, which we do with our model.

Ensuring data quality of CS data through validation (checking that the data submitted follows the required format) and verification (ensuring data quality of the CS datasets) approaches are sometimes difficult to identify species to the species level \citep{baker2021verification}. For instance, observed species are recorded at the genus level or a different level (for example "unidentified woodpecker") and during the verification process, these records are identified to the species level, as in the Bird Wasp Survey \citep{perry2021citizen}. Such possibilities have not been considered in the existing model frameworks that account for misclassification in SDMs used for modelling CS observations. We therefore propose a flexible and general framework that allows inter-taxonomic (mis)classification such as species - genus (mis)classification to be accounted for. 

Another pending question of interest is whether the true species identity of the CS observations can be predicted. Recent approaches aimed at solving this problem have used deep learning \citep{suzuki2022deep, saoud2020miss, lotfian2021partnership, willi2019identifying,keshavan2019combining} and generalised linear (mixed) models \citep{tiago2017using}. These methods do not take into account the classification probabilities in their predictions, and as a consequence cannot account for predictions that are well out of its range. Moreover, some of the machine learning algorithms do not provide uncertainty estimates for their predictions. Our proposed model framework makes it possible to continually update the information of the verification of observed species by taking into account the estimated classification probabilities from available verified identifications in the prediction of the true species identity of the observed species. This can help in the identification of individuals and flag potential misclassifications, for example, if an individual is misidentified as being well out of its range.

Here we present a method that explicitly estimates misclasification probabilities together with abundance or occupancy estimates, as well as trying to classify an observation as the correct species. The method we present needs data with both an observation and verification. These verification data can be from automated approaches such as Machine learning algorithms such as Artsorakel \citep{Artsorakel} or by human experts such as community verification for iNaturalist data \citep{matheson2014inaturalist}.  Here we view the classifications (either by ML or community verification) as a verified data and use our method to account for the misclassification in the CS observations. The additional verified data  makes the estimation of the misclassification probabilities identifiable like any other occupancy or abundance model \citep{chambert2015modeling, wright2020modelling}. We also predict the "true" species identity of the CS observations by taking into account the estimated classification probabilities. The prediction can help speed up the verification process by flagging potential misidentifications that need further verification by experts once a citizen scientist reports an observation.

\section{Methodology}
\label{section:methodology}

\subsection{Model framework}
The proposed model framework assumes that each observation is of an individual with a true state (usually unknown) and observed state (\textbf{Y}) (where the sets of possible states do not have to be the same), and for that observation there is a verified state (\textbf{V}) which we assume to represent the "true" state \citep{clare2019making}.

\subsubsection{Misclassification}
We assume that over a given study region $D \in \mathbb{R}^2$, there are $i = 1, 2, \ldots , R$ indexed locations, where each location has only one of the individuals. These individuals, reported as $k=1, 2, \ldots, K$ categories, can be verified to any $s=1,2, \ldots, S$ states. The reported categories could be on any taxonomic level, depending on the ability of the citizen scientist, from the species level to the kingdom level, partial identifications or unidentified groups. The verified state could also be on any taxonomic level, depending on the available information for the verification process. The reported categories and the observed states are not necessarily the same, and we use categories and states to project this difference throughout the paper.

Let $\Omega_{sk}$ be the probability that a single verified state $s \in \{1, \ldots, S \}$ is classified as category $k \in \{1, \ldots, K \}$. The probabilities across all the possible $k$ categories sum to $1$. Generally, the confusion matrix for the classification can be expressed as:
\begin{equation}
\mathbf{\Omega} = 
 \begin{bmatrix}
\Omega_{11} & \Omega_{11}& \cdots & \Omega_{1k}& \cdots& \Omega_{1K}   \\
\Omega_{21} & \Omega_{22}& \cdots& \Omega_{2k}& \cdots& \Omega_{2K} \\
\vdots & \vdots & \cdots& \vdots & \cdots& \vdots\\
\Omega_{s1} & \Omega_{s2}& \cdots& \Omega_{sk}& \cdots& \Omega_{sK} \\
\vdots & \vdots & \cdots& \vdots & \cdots& \vdots\\
\Omega_{S1} & \Omega_{S2} & \cdots & \Omega_{Sk}& \cdots& \Omega_{SK} \\
\end{bmatrix}   
\end{equation}
where the rows correspond to the verified states $s$ and the columns correspond to the reported categories $k$. 

For example, a set of hypothetical ornithological reportings could have four verified states: black woodpecker, pileated woodpecker, yellow-bellied sapsucker and Williamson's sapsucker. As well as being reported at the species level, more general classifications can be used. For example, the North American Breeding Bird Survey also includes "unidentified Sapsucker", "unidentified Woodpecker", and four different Northern Flickers \citep{sauer2013north}. An example of the classification probability (confusion matrix) is shown in Table \ref{example}. 

\begin{table}[h!]
\centering
\begin{tabular}{||m{10em} | m{5em}  m{5em} m{5em}  m{5em}||} 
\hline
& & \textbf{Observed state} & & \\

 \textbf{Verified state} & black  woodpecker & woodpecker & sapsucker & Unidentified  woodpecker \\ [0.5ex] 
 \hline\hline
black woodpecker & 0.8 & 0.1 & 0.1 & 0 \\ 
pileated woodpecker & 0.05 & 0.7 & 0.2 & 0.05 \\
 yellow-bellied sapsucker & 0 & 0.9 & 0 & 0.1 \\
 williamson's sapsucker & 0 & 0 & 1 & 0 \\ [1ex] 
 \hline
\end{tabular}
\caption{Example of confusion matrix that is applicable to our model.}
\label{example}
\end{table}

\subsubsection{Distribution models}
 We also assume that these locations are the realisations of the point pattern which is characterised by the mean intensity \citep{cressie2015statistics}. 
Here we model the mean intensity $\lambda_{is}$ of the true state $s$ as an inhomogeneous point process (PPM) which assumes that the data are dependent on the environment covariate,  or as a log-Cox Gaussian Point process (LGCP) where we assume a spatial dependency in the data \citep{renner2015point}. The mean intensity of the verified observations (\textbf{V}) is modelled using the inhomogeneous  point process and defined as:

\begin{equation} \label{intensity}
 \ln (\lambda_{is})= \beta_{0s} +  \mathbf{\beta}'_{s}  \textbf{x}  ,
\end{equation}
where $\beta_{0s}$ is the intercept of verified state $s$, $\beta_{s}$ is the vector of covariate effect and $\textbf{x}$ is the covariate that affects the observation of the verified (true) states.

Let $p_{is}$ be the probability of obtaining verified state $s$ at location $i$. Estimating these probabilities from the mean intensities of the states, 

\begin{equation}\label{proportion}
    p_{is} = \frac{\lambda_{is}}{\sum_{s}\lambda_{is}},
\end{equation}
where $\lambda_{is}$ is given by \eqref{intensity}. 

The verified states $s = 1,2,\ldots, S$ at location $i=1,2,\ldots,R$ is then a realisation from a categorical distribution with probability $p_{is}$. This particular specification of the model for the true states is  multinomial logit regression model used for categorical variables (See Supplementary information 1).

Given which verified state was present, the reported category at location $i$, $Y_i$, is a draw from $K$ categories with probability $\Omega$.\\

\begin{equation}
    Y_i|V_{\cdot i} \sim \text{Categorical}(\Omega_{\cdot,k}),
\end{equation}
where $\Omega_{\cdot,k}$ refers to the probability of being classified as any of the $K$ categories given which verified state was present at location $i$. 

The hierarchical likelihood of the model proposed is given as follows:
\begin{equation*}
    \begin{split}
        \ln (\lambda_{is}) &= \textbf{x}'\beta \\
        p_{is} &= \frac{\lambda_{is}}{\sum_i \lambda_{is}}\\
        V_{i} | p_{is} & \sim Categorical (p_{i.})\\
        Y_i | V_{i}& \sim Categorical(\Omega_{V_i, \cdot})
    \end{split}
\end{equation*}
for $s= 1, \ldots, S$ verified states, $k=1,2,\ldots, K$ reported categories and $i=1, 2, \ldots,R$ number of sites.

\subsection{Generalisation of model framework}
The proposed framework generalises the existing multi-species distribution models that account for false positives. Given our specification of model framework, our model is connected to that of \cite{wright2020modelling} by using the relationship between the multinomial and the Poisson distribution \citep{steel1953relation} as well as using a species by species confusion matrix (Supplementary information 2). By extending the model proposed by \cite{wright2020modelling}, our model framework can also be seen as a generalisation of the works by \cite{chambert2018two}, \cite{chambert2015modeling} and \cite{chambert2018new}. 

\subsection{Predicting true states abundance}
The true states can also be predicted from the estimates of $\mathbf{\Omega}$ to check whether we obtain each true state intensity and abundance map and to explore how the relationship between the observed and true states changes with the environmental changes (which only affects the true distributions). With this result, species abundance maps for regions yet to be covered could be predicted from available CS data and the classification probabilities.

Let $\Gamma_{iks}$ be the probability that the true (verified) state is $s$ given that category $k$ was observed at site $i$. From Bayes theorem,

\begin{equation}
\label{pred true}
    \Gamma_{iks} = \frac{\text{P(reported = k|verified = s) P(verified=s)}}{\sum_{s}\text{P(reported = k|verified = s) P(verified=s)}}= \frac{\hat \Omega_{sk}\times \hat p_{is} }{\sum_{s} \bigg [ \hat \Omega_{sk}\times \hat p_{is} \bigg]},
\end{equation}
where $\hat \Omega_{sk}$ is the estimated probability of reporting category $k= 1,2, \ldots ,K$ given the verified state $s$ and $\hat p_{is}$ is the estimated probability for verified species $s = 1,2, \ldots, S$ and $i=1,2,\ldots,R$ indexed sites.

Reported observation category $k$ at location $s$ from Citizen Scientists can be flagged for further verification if the posterior predicted probability  $\Gamma_{iks}$ is very low.
\textit{The predicted true states can be chosen as the species with the maximum of the probability $\Gamma_{iks}$ for all verified states $i= 1,2, \cdots ,S$. Alternatively, the true states can be simulated from Categorical distribution with probability ($\Gamma_{k.j}$) for the reported categories $k= 1,2, \cdots ,K$ at location $j$. Thus, the predicted true state depends on the estimates of \textbf{$\Omega$} and the predicted mean intensity of each state at the location $j$}.

\subsection{Simulation Study}
To demonstrate how our model works and its use in prediction, we performed a simulation study for $S=3$ verified states and $K=4$ reported categories over $R=400$ indexed sites. A single covariate was used and was generated uniformly over the domain $[-1,1]$. The true intensity was simulated from equation \eqref{intensity}. The intercept of the model for the three verified states were chosen as $\beta_{01} =-1$, $\beta_{02} =1$, and $\beta_{03} =0$. The environmental covariate effect for each verified state was chosen as $\beta_{11}= 2$, $\beta_{12}= 0$ and $\beta_{13}= -2$. The intercept and covariate effect for the three verified states were carefully chosen such that they have a sum to zero constraint, and all species would have a location where they are more probable to occur. The range of covariate values with the probability of observing a verified (true) state $i$ from our parameter values chosen is shown in Figure \ref{fig:covariate}.

\begin{figure}[htbp]
    \centering
\includegraphics[scale= 0.079]{Supplementary figures/covariates.png}
\caption{Probability of verified (true) states from the simulation study parameter choices over the given covariate domain.}
    \label{fig:covariate}
\end{figure}

The confusion matrix used for the simulation study is presented in Table \ref{confusion matrix simulation}. The values were chosen such that it is impossible to misclassify state $3$ as category $1$ or $2$. 
\begin{table}[h!]
\centering
\begin{tabular}{||c| c c c c||} 
\hline
& & \textbf{Observed category} &  & \\
 \textbf{Verified states} & 1 & 2& 3 & 4 \\ [0.5ex] 
 \hline\hline
1 & 0.7 & 0.05 & 0.13 & 0.12\\ 
2 & 0.10 & 0.80 & 0.05 & 0.05\\
3 & 0 & 0 & 0.9 & 0.10\\ [1ex] 
 \hline
\end{tabular}
\caption{The classification probabilities (confusion matrix) used in the simulation study.}
\label{confusion matrix simulation}
\end{table}

The simulation was repeated 1000 times, and for each run the true intensity was simulated using the same parameters as defined above. This was done to ensure that the results analysed would not be due to randomness.

%\subsection{Fitting the model}
\subsubsection{Fitting the model and estimating the parameters}
The model was fitted with MCMC using the Bayesian modelling framework. All the analyses were done using $R$ software  \citep{chambers2008software}. The mcmc was run with the nimble package \citep{de2017programming}. The priors for $\beta_{0i}$ and $\beta_{1i}$ for $i = 1, 2, \cdots, S$ states were chosen from a normal distribution with mean $0$ and standard deviation of $1$, i.e. $ \beta_{0i} \sim N(0, 1)$ and $ \beta_{1i} \sim N(0, 1)$. The priors of the confusion matrix ($\mathbf{\Omega}$) were chosen from the Dirichlet distribution with parameter alpha equal to $1$.

The chains were run for $5 \times 10^5$ number of iterations for $3$ chains, and the first $2 \times 10^5$ iterations were chosen as the burn-in. The fitted model was ignored when the model did not converge (looking at trace plots and with a Gelman statistic value greater than 1.04 \cite{brooks1998general}), showed an error in the running of the model as well as having a small effective sample size. The convergence was done with the 'ggmcmc' package \citep{fernandez2016ggmcmc} in $R$. 

To check how well we estimated the parameters in the model, the model parameters $\mathbf{\beta_0}$, $\mathbf{\beta_1}$ and $\mathbf{\Omega}$ were evaluated by estimating the root mean squared error (RMSE) and coverage of the estimated parameters. Better results would be parameters with lower RMSE and higher coverage. The results were presented with the 'ggplot' package \citep{wickham2016package} in $R$.

\subsection{Application to data}
We demonstrate application of the model using a butterfly dataset that was downloaded from iNaturalist. iNaturalist is a Citizen Science platform that hosts over ninety million occurrence observations with well over a million observers (Website https://www.inaturalist.org/ visited on 18th March 2022). Observers collect occurrence records and upload their observations with images, sounds and other valuable information that allow for verification \citep{matheson2014inaturalist}. The species name provided by the observer is known as the species guess or reported species. The observations reported goes through a community verification, and is accepted when two-thirds of users verifying the observation agree upon the taxon identification \citep{ueda2020inaturalist}. Community verified observations are termed "research grade", and we will in the following refer to these observations as the true species. Observations without community verification are termed as "needs id".

The butterfly data used for the demonstration was collected from United States of America in the period from 2019 to 2020. Specifically we selected the butterfly species: the viceroy (\textit{Limenitis archippus}), the queen butterfly (\textit{Danaus gilippus}) and the monarch butterfly (\textit{Danaus plexippus}). Any other species apart from \textit{Limenitis archippus} in the genus \textit{Limenitis} was re-coded as "other Limenitis", other species in the \textit{Danaus} genus was also re-coded as "other Dananus" and any other species outside these species categories were denoted as "other". The distribution of the species to be analysed are presented in Figure \ref{fig:data}.

\begin{figure}[htbp]
    \centering
\includegraphics[scale= 0.36]{Supplementary figures/data_plot_new.png}
\caption{The subset of the butterfly dataset downloaded from iNaturalist used for the analysis. The data are faceted according to the true species name and coloured according to the reported category.}
    \label{fig:data}
\end{figure}

Climatic factors such as precipitation, temperature and elevation of the area are major drivers behind the population dynamics of the North American Monarch butterfly \citep{brym2020prevalence}. The butterfly has an annual multigenerational migration cycle and for every fall, those at the Rocky Mountains travel great distances to the summer breeding grounds, where most of them aggregate \citep{culbertsonlong}. \cite{culbertsonlong} noted that climatic changes affects this migration as \cite{zipkin2012tracking} adds that this is a major driver in its population dynamics. The queen butterfly and viceroy butterfly are co-mimics and have great resemblance because of their patterns \citep{prudic2019mimicry, ritland1991revising}.This suggests that the abundance of one of them affects the other in the location.

We developed a spatial model where we used elevation from the Bioclim data in the raster package \citep{hijmans2013raster}, month, number of agreements and number of disagreements as covariates. The true intensity of the verified species were estimated using INLA \citep{rue2019inla} and the classification probabilities in nimble \citep{de2017programming}. The details can be found in the code in the Supplementary information.

The true species for the data that needed verification in 2019 was predicted by retrieving the species with the highest posterior predicted probability. Butterfly data for the states of Florida, Montana, Minnesota, Wisconsin, Illinois and Indiana in 2020 were selected and the true species for both the data that needed verification and those with community verification were predicted by retrieving the species with the highest posterior predicted probability.

\section{Results}

\subsection{Simulation study}

\subsubsection{Intensity of verified states}
Table \ref{reults_simulation} presents the estimates of the parameters from the 1000 simulations summarised by using the median, root mean square error (RMSE) and the coverage. The contrast in the estimates, using state $1$ as the reference state, were less biased with a small root mean square error and high coverage as can be observed from Table \ref{reults_simulation}. This is what we expected considering that the multinomial logit regression was used for the verified states.  

\begin{table}[htbp]
    \centering
    \begin{tabular}{||p{3cm}|p{1.5cm}p{2cm}p{2.0cm}p{1.5cm}p{0cm}||}
    \hline
\centering Parameters & \centering True value &\centering Estimate &\centering RMSE &\centering Coverage &\\ \hline \hline
\centering $\beta_{02} - \beta_{01}$  &\centering 2 &\centering 1.89 &\centering 0.046 & \centering 0.94&\\ 
\centering $\beta_{03} - \beta_{01}$  &\centering 1  &\centering  0.91 &\centering 0.058 & \centering 0.96&\\  
\centering $\beta_{12} - \beta_{11}$ &\centering -2 &\centering  -1.76 &\centering 0.058 &\centering 0.97&\\ 
\centering $\beta_{13} - \beta_{11}$& \centering -4 &\centering -3.67 &\centering 0.1471 & \centering 0.91 &\\ \hline
\centering  $\Omega_{11}$ &\centering $0.7$ &\centering $0.69$ &\centering $3.8 \times 10^{-3}$ & \centering 0.94&\\ 
 \centering $\Omega_{21}$ &\centering 0.10 &\centering 0.10 &\centering $3.63 \times 10^{-4}$ & \centering 0.95&\\ 
 \centering $\Omega_{31}$ &\centering 0.00 &\centering 0.00 &\centering $1.6 \times 10^{-9}$ &\centering $-$ &\\
  \centering $\Omega_{12}$ &\centering 0.05 &\centering 0.05  &\centering  $8.26 \times 10^{-4}$ & \centering 0.92&\\
 \centering $\Omega_{22}$ &\centering 0.80 &\centering 0.79 &\centering $6.66 \times 10^{-4}$ &\centering 0.96&\\
  \centering $\Omega_{32}$ &\centering 0.00  &\centering 0.00 &\centering $1.60 \times 10^{-9}$ &\centering - &\\ 
 \centering $\Omega_{13}$  &\centering  0.13&\centering 0.13 &\centering  $1.84 \times 10^{-3}$ &\centering 0.96&\\
\centering $\Omega_{23}$ &\centering 0.05 &\centering 0.05 &\centering  $2.21 \times 10^{-4}$ &\centering 0.95&\\ 
 \centering $\Omega_{33}$   &\centering 0.90 &\centering 0.9 &\centering  $7.28 \times 10^{-4}$ &\centering 0.97&\\ 
 \centering $\Omega_{14}$ &\centering 0.12 &\centering 0.12 &\centering  $1.99 \times 10^{-3}$ &\centering 0.93&\\ 
 \centering  $\Omega_{24}$  &\centering 0.05 &\centering 0.05 &\centering  $2.09 \times 10^{-4}$ &\centering 0.96&\\ 
  \centering $\Omega_{34}$ &\centering 0.10 &\centering 0.10 &\centering  $7.13 \times 10^{-4}$ &\centering 0.97 &\\ \hline
    \end{tabular}
    \caption{True values and posterior summaries of estimates of parameters from the simulation study. There are no coverage values for $\Omega_{31}$ and $\Omega_{32}$ because the true value can never be within the confidence interval. All the results are converted to two decimal places.}
    \label{reults_simulation}
\end{table}


\subsubsection{Classification probabilities}
Table \ref{reults_simulation} provides estimates of the parameter of interest, the classification probabilities ($\Omega$). The estimates of classification probabilities were almost unbiased with a small root mean square error and higher coverage for most cases. Even though we obtained relative abundances for the verified states as discussed above, the model proposed provides precise and accurate estimates of the classification probabilities. This suggests that the estimation of the classification probabilities is somewhat independent of the model for the intensity or verified species. So one can estimate the classification probability precisely and accurately for any given distribution model the verified species takes. 

\subsubsection{Predicting the verified states}

As explained in Section 2 above, the true verified states can be predicted from the reported states and the classification probabilities. The posterior probability of verified states $s$ given the reported category is shown in Figure \ref{fig:results2} , for $i=1,2,3$ and $K= 4$ categories.  

\begin{figure}[htbp]
    \centering
\includegraphics[scale= 0.1]{Supplementary figures/results_sub.png}
\caption{The figure shows the predicted posterior probability of observing verified states  given that reported category is a) category 1,  b) category 2, c) category 3 and d) category 4. The green shaded colour shows the region of coverage for the posterior probability of species 1, red colour for species 2 and blue colour for species 3.}
    \label{fig:results2}
\end{figure}

 The results in Figure \ref{fig:results2} showed that the posterior probability of identifying any of the verified states depends on the location of the state as well as the its misclassification probabilities. For example, assuming that category $1$ is reported, the posterior probability curve of the state $1$ was shifted down since it has a higher probability of being the true state over the entire covariate range and suggesting an impossibility for the reported category to be verified state $3$ (from Figure \ref{fig:results2} a)), even for regions where true state $3$ was higher in the true simulation in Figure \ref{fig:covariate}. Similar deductions can be made when categories $2$, $3$ and $4$ were reported.

\subsection{Data Application}
The results for the classification probabilities and the parameters of the model are presented in the Supplementary information. Although the viceroy and the queen are co-mimics \citep{ritland1991revising}, the misclassification for reporting viceroy as queen butterfly and the converse was negligible, suggesting that the citizen scientists were able to distinguish between them. 

\begin{figure}[htbp]
    \centering
\includegraphics[scale= 0.60]{Supplementary figures/misclassification_data_plot.png}
\caption{Percentage of correct classification for the data that needed verification in 2019 ("need id 2019") and 2020 ("need id 2020") and those with research grade in 2020 ("research 2020) before (deep blue colour) and after (light blue colour) the posterior prediction of the true species. The percentages for each category are presented in their corresponding bars.}
    \label{fig:percentage_pred}
\end{figure}

The proportion of correct classification for the true species identity that needed verification in 2019 increased from 70.73\% before prediction to 100\% after the posterior prediction with the model, as can be seen from Figure \ref{fig:percentage_pred}. The proportion of correct classification for the species that needed verification in 2020 increased from 66.67\% before prediction to 100\% after the prediction (Figure \ref{fig:percentage_pred}). For the data with verified true species identity, there was a 0.5\% increase from prediction using our model(Figure \ref{fig:percentage_pred}).

\section{Discussion}
The current study has provided a general framework to account for misclassification in the multi-species distribution models. The model can be used to predict the true species, and how this prediction depends on the misclassification probabilities and the actual distribution.

The simulation study demonstrated that if we think we have observed a species that is difficult to identify, what it actually is will depend on where we observe it. This matches the behaviour of ornithologists when asked to identify a bird from a photo: their first question is usually "where was the photograph taken?" (GrrlScientist, \textit{pers. comm})

With the model for the true intensity (equation \eqref{intensity}) being a multinomial logit model, the model returned the contrasts of the estimates of the parameters relative to a reference species. Thus, any model that is assumed for the generation of the verified states, such as point processes, etc as well as any model for estimating the ecological parameters such as joint species distribution models should be feasible for this framework.

Following from the argument in the previous paragraph, the model framework proposed here can be used to identify probable misidentifications, by flagging observations that are improbable of being correctly classified. Our simulation study showed that in real word situations, if the species are relatively likely to occur in a region, the posterior probability favours the species with the highest classification in that reported category, and the vice versa.  Thus we can not only flag that a species may be misidentified (if the identification has a low probability of being correct), but we can also suggest the correct identification. With the large number of observations coming into data portals such as iNaturalist, a model such as ours can form the basis of automated screening of observations, to identify those which might need manual checking.  

Our simulation study stressed on the importance of accounting for misclassification in multi-species models just as was noted in previous literature \citep{chambert2015modeling,kery2020applied}. The posterior predicted probability for the reported states heavily relies on the weights from the misclassification probability. Failure to account for that would mean our posterior probability would be the same as the probability of the verified state. This would lead to the underestimation of the prediction of the ranges of the coverage and possibly abundance in the verified states \citep{molinari2012monitoring}.

The model framework proposed does not just account for misidentifications, but identifications at different taxonomic levels. This implies that CS data analysts can make use of more data, especially when the data have some missing identifications for a taxonomic level, which will sometimes be more informative. We have shown that our model can improve an identification based on the location, for example, an unidentified butterfly from our data is unlikely to be a queen butterfly if it is observed in Wisconsin, because queen butterfly is not found in that state.

Our model showed a 29\% increase in the number of correct identifications for the data that needed verification in 2019, 33\% increase in the number of correct identifications for the data that needed verification in 2020 and a non-significant increase in 2020 for data with community verification. Although the queen and viceroy butterflies have a greater resemblance between their ventral patterns and co-mimic each other \citep{ritland1991revising}, citizen scientists appeared to be able to correctly classify these two species for all the months. Although the model proposed was able to predict the true species given the reported category to a higher degree, we suggest that the community verification is a necessity to get the true species information.

The model framework is flexible and can be generalised into any joint species distribution models. Although we use a point process model for the true distribution, our misclassification model can be plugged into similar model that estimates either abundance or incidence. And because our model does not assume the true states are the only possible reported states, it allows for a lot of flexibility in what is reported (for example, it could be developed to take DNA sequences and match them to species). This will make it possible to analyse Citizen Science data alongside other data sources to account for misclassification at any level in the data collection process. 



